Leaping through tree space: continuous phylogenetic inference for rooted and unrooted trees

Phylogenetics is now fundamental in life sciences, providing insights into the earliest branches of life and the origins and spread of epidemics. However, finding suitable phylogenies from the vast space of possible trees remains challenging. To address this problem, for the first time, we perform both tree exploration and inference in a continuous space where the computation of gradients is possible. This continuous relaxation allows for major leaps across tree space in both rooted and unrooted trees, and is less susceptible to convergence to local minima. Our approach outperforms the current best methods for inference on unrooted trees and, in simulation, accurately infers the tree and root in ultrametric cases. The approach is effective in cases of empirical data with negligible amounts of data, which we demonstrate on the phylogeny of jawed vertebrates. Indeed, only a few genes with an ultrametric signal were generally sufficient for resolving the major lineages of vertebrates. Optimisation is possible via automatic differentiation and our method presents an effective way forwards for exploring the most difficult, data-deficient phylogenetic questions.

==> diff/03_diff.tex <==
Phylogenetic inference, the task of reconstructing the evolutionary relationships across taxonomic units given observational data, has a wide range of theoretical and practical applications in \DIFdelbegin \DIFdel{the biological sciences}\DIFdelend \DIFaddbegin \DIFadd{biology}\DIFaddend , such as \DIFdelbegin \DIFdel{in biology}\DIFdelend \DIFaddbegin \DIFadd{evolution}\DIFaddend ~\parencite{cavalli1967, felsenstein2004, omeara2012}\DIFaddbegin \DIFadd{, conservation~}\parencite{rolland_cadotte} \DIFaddend and epidemiology~\DIFdelbegin %DIFDELCMD < \parencite{Grenfell2004-yl}%%%
\DIFdelend \DIFaddbegin \parencite{Grenfell2004-yl, faria2021}\DIFaddend , but also in \DIFaddbegin \DIFadd{comparative }\DIFaddend linguistics~\parencite{mace2005} and cultural anthropology~\parencite{collard2006, morrison2014}. In particular, the COVID-19 pandemic has catalysed \DIFdelbegin \DIFdel{research efforts to develop efficient }\DIFdelend \DIFaddbegin \DIFadd{the development of efficient phylogenetic }\DIFaddend tools and methods \DIFdelbegin \DIFdel{in phylogenetics}\DIFdelend \DIFaddbegin \DIFadd{to better understand the virus' origin, spread, and evolution}\DIFaddend ~\parencite{lemoine2021, otoole2021, attwood2022, sanderson2022, turakhia2022, voznica2022, demaio2023}. For biological problems, tree inference is primarily informed by molecular sequence data (i.e., nucleotide or amino acid sequences), for which an extensive body of literature exists~\parencite{sanderson2002, yang2006, yang2012}. Other \DIFdelbegin \DIFdel{sources }\DIFdelend \DIFaddbegin \DIFadd{types }\DIFaddend of biological data such as morphology~\parencite{Lee2015-es}, fossils~\parencite{Morlon2011-pe}, and auditory communication in animals~\parencite{arato2021} can also be used as input.
\DIFdelbegin \DIFdel{Yet despite an explosion in data available for millions of taxonomic units, as seen during the recent pandemic, we are still unable to effectively explore the gigantic parameter spaces involved during inference.
}\DIFdelend 

Two key parameters considered when inferring a phylogenetic tree include the \emph{topology}, the branching pattern that specifies the evolutionary relationships between operational taxonomic units, and \emph{branch lengths}, the amount of evolutionary divergence that occurred between the branching events. A substantial amount of research has been conducted on how to parameterise branch lengths~\parencite{bromham2003, dosreis2016}, especially through the use of \DIFaddbegin \DIFadd{various }\DIFaddend molecular clocks~\parencite{zuckerkandl1962}. \DIFdelbegin \DIFdel{Conversely, relatively little }\DIFdelend \DIFaddbegin \DIFadd{Similarly, although to a lesser degree, }\DIFaddend progress has been made on methods for \DIFdelbegin \DIFdel{exploring the massive spaces of possible tree topologies. This is a fundamental challenge for inference given }\DIFdelend \DIFaddbegin \DIFadd{efficient exploration of the space of tree topologies}\parencite{stamatakis2014}\DIFadd{, which is fundamentally challenging due to }\DIFaddend its combinatorial complexity\DIFdelbegin \DIFdel{: }\DIFdelend \DIFaddbegin \DIFadd{. Indeed, }\DIFaddend for $n$ taxa, there are $(2n-3)!!$ possible rooted tree arrangements\DIFdelbegin \DIFdel{. This means that }\DIFdelend \DIFaddbegin \DIFadd{, where $n!!$ denotes the semifactorial of $n$ --- }\DIFaddend even a small dataset of \DIFdelbegin \DIFdel{10 }\DIFdelend \DIFaddbegin \DIFadd{ten }\DIFaddend taxa can be enumerated by 34 million unique rooted trees. Moreover, finding the \DIFaddbegin \DIFadd{global }\DIFaddend optimal tree is NP-hard for all major optimality criteria (e.g., maximum parsimony~\parencite{foulds1982}, minimum evolution~\parencite{day1986}, maximum likelihood~\parencite{roch2006}). Methods such as linear programming~\parencite{catanzaro2012} or branch and bound~\parencite{Hendy1982-dy} can provide exact solutions, but are practically limited to problems with $\approx$ 15 or fewer taxa. To overcome these challenges, the overwhelming majority of state-of-the-art software (e.g., \texttt{MrBayes}~\parencite{huelsenbeck2001}, \texttt{PAUP}~\parencite{Wilgenbusch2003-mu}, \texttt{BEAST}~\parencite{Drummond2007-za}, \texttt{PAML}~\parencite{Yang2007-ez}, \texttt{RAxML}(\texttt{-NG})~\parencite{stamatakis2014, kozlov2019}, \texttt{FastME}~\parencite{lefort2015}, \texttt{IQ-TREE}~\parencite{nguyen2015, minh2020}) rely on hand-engineered search heuristics to perform tree topology optimisation \DIFdelbegin \DIFdel{.
}%DIFDELCMD < 

%DIFDELCMD < \input{fig/fig1}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{The most popular of these methods still have several limitations, and this includes heuristics }\DIFdelend \DIFaddbegin \DIFadd{or Bayesian analysis. These are traditionally }\DIFaddend based on subtree pruning and regrafting (SPR) and tree bisection and reconnection (TBR) operations, which have empirically been shown to be the best available methods for exploring tree topology space~\parencite{stamatakis2014, Park2010-zq}.
\DIFdelbegin \DIFdel{First, the computational cost of such heuristic approaches scales poorly as the number of taxa increases. For instance}\DIFdelend \DIFaddbegin 

\DIFadd{However, such methods still have limitations. First, hill climbing using heuristic approaches necessitates multiple evaluations of the objective function to pick the best move. While these heuristics are still polynomial}\DIFaddend , exhaustive exploration of single SPR operations is quadratic in complexity, and paired \DIFdelbegin \DIFdel{changes is quartic. The computational cost of SPR is further compounded by large memory requirements for tracking the changes from one iteration to the next. }\DIFdelend \DIFaddbegin \DIFadd{operations (two sequential SPR changes) are quartic. }\DIFaddend Second, all the aforementioned tree arrangements are prone to \DIFdelbegin \DIFdel{convergence to poor local minima}\DIFdelend \DIFaddbegin \DIFadd{being trapped in local optima and even if a global optimum is found, terraces of trees with identical quality exist}\DIFaddend ~\parencite{sanderson2011}\DIFdelbegin \DIFdel{due to the inability of heuristic operations to provide sufficient directions of change to a better tree}\DIFdelend . This phenomenon is exacerbated when concatenating multiple genes in \DIFdelbegin \DIFdel{a supermatrix approach~}%DIFDELCMD < \parencite{rokas2003, dequeiroz2007}%%%
\DIFdel{, and }\DIFdelend \DIFaddbegin \DIFadd{supermatrices~}\parencite{rokas2003, dequeiroz2007, Chernomor2016-vi} \DIFadd{or }\DIFaddend when using genomic-scale \DIFdelbegin \DIFdel{data sets that lead to further computational demands}\DIFdelend \DIFaddbegin \DIFadd{datasets which require extensive computational resources}\DIFaddend .

\DIFdelbegin \DIFdel{We }\DIFdelend \DIFaddbegin \DIFadd{To }\DIFaddend address these shortcomings\DIFdelbegin \DIFdel{by proposing a new paradigm }\DIFdelend \DIFaddbegin \DIFadd{, we propose }\textsb{\DIFadd{GradME}}\DIFadd{, a new direction }\DIFaddend for tree topology inference \DIFdelbegin \DIFdel{, expanding }\DIFdelend \DIFaddbegin \DIFadd{which expands }\DIFaddend the problem space using a continuous rather than discrete parameterisation of a phylogenetic tree. \DIFdelbegin \DIFdel{To our knowledge}\DIFdelend \DIFaddbegin \DIFadd{Generally}\DIFaddend , aside from considering metrics (e.g., distances in tree space)~\DIFdelbegin %DIFDELCMD < \parencite{St_John2017-vq,Dinh2017-og,Billera2001-il}%%%
\DIFdelend \DIFaddbegin \parencite{St_John2017-vq,Dinh2017-og,Billera2001-il,Chernomor2016-vi}\DIFaddend , performing topological search in a continuous tree space has \DIFdelbegin \DIFdel{not been attempted}\DIFdelend \DIFaddbegin \DIFadd{rarely been explored (for recent work in hyperbolic spaces, see~}\parencite{matsumoto2021, wilson2021, macaulay2023, mimori2023}\DIFadd{)}\DIFaddend . Furthermore, very few approaches have made use of gradient-based tree proposals~\DIFdelbegin %DIFDELCMD < \parencite{zhang2018, nesterenko2022,Dinh2017-og}%%%
\DIFdelend \DIFaddbegin \parencite{matsumoto2021, zhang2018, nesterenko2022,Dinh2017-og}\DIFaddend . Although maximum likelihood and Bayesian inference criteria are more popular and generally considered state-of-the-art~\parencite{huelsenbeck2001, stamatakis2014, Drummond2007-za, minh2020, Wilgenbusch2003-mu, ayres2012}, \DIFdelbegin \DIFdel{our }\DIFdelend \DIFaddbegin \DIFadd{the GradME }\DIFaddend framework optimises tree topology under a balanced minimum evolution (BME) criterion~\parencite{Pauplin2000-vk,Desper2002-uy} using \DIFdelbegin \DIFdel{dissimilarity }\DIFdelend \DIFaddbegin \DIFadd{distance }\DIFaddend matrices as an input. This criterion is well-principled~\parencite{Kidd1971-sk} \DIFdelbegin \DIFdel{theoretically can match the performance of maximum likelihood approaches~}%DIFDELCMD < \parencite{Roch2010-uj}%%%
\DIFdel{. This }\DIFdelend \DIFaddbegin \DIFadd{but generally performs worse than likelihood-based~}\parencite{price2009, yang2012, lefort2015}\DIFadd{. However, the }\DIFaddend framing of the minimum evolution criterion~\parencite{Kidd1971-sk, Rzhetsky1992-qj} has \DIFdelbegin \DIFdel{also }\DIFdelend been proven to be statistically consistent~\parencite{Desper2004-ij,felsenstein2004} and has repeatedly shown \DIFdelbegin \DIFdel{outstanding performance in a range of }\DIFdelend \DIFaddbegin \DIFadd{good (although not state-of-the-art) performance in various }\DIFaddend settings~\parencite{Kuhner1994-cf, kumar2000, Gascuel2006-sr, lefort2015}. 

To better explore the space of possible trees, we expand the space over which we need to search. \DIFdelbegin \DIFdel{Consequently, we use a continuous }\DIFdelend \DIFaddbegin \DIFadd{Our novel vector }\DIFaddend representation of a phylogenetic tree\DIFaddbegin \DIFadd{, Phylo2Vec}\DIFaddend ~\parencite{penn2023}\DIFdelbegin \DIFdel{to greatly }\DIFdelend \DIFaddbegin \DIFadd{, has a natural continuous extension, allowing us to }\DIFaddend improve the ability to search parts of this space. Appealing to a common analogy that casts the optimal tree search problem as finding a needle in a haystack, our approach observes a much bigger haystack, but the hay is in very large bundles, many of whom have a needle, and for these bundles we have access to a (weak) magnet. Providing details to this analogy, the size of the usual phylogenetic haystack with $n$ taxa is $(2n-3)!!$~\parencite{Felsenstein1978-qc}, while we search a much larger haystack of size $(n!)^2$. There are $n!$ bundles in this larger haystack, each of which contains $n!$ trees, but for any tree, $2^{n-1}$ bundles will contain that tree. Although the proportion of bundles containing a needle shrinks exponentially, we propose a novel approach (Queue Shuffle) that chooses bundles that should be closer to one with a needle. For any given bundle, we also introduce a continuous objective function that can be efficiently traversed using gradient descent approaches (the weak magnet) developed for large-scale machine learning problems~\parencite{Kingma2014-ow, loshchilov2018, shazeer2018}. This continuous objective facilitates enormous changes to tree topology in a single step in a direction that improves the objective function. After searching any given bundle using the continuous objective, we use Queue Shuffle, which improves the switch towards the next bundle to search. \DIFdelbegin \DIFdel{Our counterintuitive approach , called GradME, offers a powerful alternative }\DIFdelend \DIFaddbegin \DIFadd{This counterintuitive approach offers a new addition }\DIFaddend to the existing heuristic methods used for topological inference, outperforming the current state-of-the-art \DIFdelbegin \DIFdel{with an }\DIFdelend \DIFaddbegin \DIFadd{but as currently stands with a larger }\DIFaddend overall complexity comparable to neighbour joining\DIFdelbegin \DIFdel{($\mathcal{O}(n^3)$)}\DIFdelend .

==> diff/04_diff.tex <==
\DIFaddbegin \DIFadd{In the following, we describe GradME, a distance-based method for continuous phylogenetic inference of rooted and unrooted trees using gradient descent. The framework can be divided into three components: i) a continuous tree representation based on Phylo2Vec~\mbox{%DIFAUXCMD
\parencite{penn2023}}\hskip0pt%DIFAUXCMD
, a bijective integer representation of phylogenetic trees; ii) gradient-based optimisation using a continuous version of the balanced minimum evolution criterion~\mbox{%DIFAUXCMD
\parencite{Pauplin2000-vk, Desper2002-uy}}\hskip0pt%DIFAUXCMD
, iii) Queue Shuffle, a method to shuffle the integer-to-taxon mapping underlying Phylo2Vec for full tree space exploration. The overall approach works for both rooted and unrooted trees.
}

%DIF >  we propose GradME, a new approach to perform topological search in a continuous, rooted, tree space. To do so, we introduce a new objective function derived from BME for rooted trees. The approach, which still requires a distance matrix as input, relies on a continuous representation of a tree derived from Phylo2Vec to optimise the edges. Due to the representation being restricted to ordered trees, we finally introduce Queue Shuffle, a method to change orderings for full tree space exploration.

\subsubsection*{\DIFadd{Balanced minimum evolution}}\DIFadd{~Popular objective functions to infer the optimal tree from phylogenetic data include maximum parsimony~\mbox{%DIFAUXCMD
\parencite{Fitch1967-dr}}\hskip0pt%DIFAUXCMD
, maximum likelihood~\mbox{%DIFAUXCMD
\parencite{felsenstein1983} }\hskip0pt%DIFAUXCMD
and minimum evolution~\mbox{%DIFAUXCMD
\parencite{Saitou1987-wg}}\hskip0pt%DIFAUXCMD
. Maximum likelihood and minimum evolution are provably statistically consistent~\mbox{%DIFAUXCMD
\parencite{Desper2004-ij,felsenstein2004}}\hskip0pt%DIFAUXCMD
, whereas maximum parsimony can be inconsistent under certain conditions~\mbox{%DIFAUXCMD
\parencite{Felsenstein1978-jt}}\hskip0pt%DIFAUXCMD
. For small to moderate sized phylogenies, methods based on maximum likelihood (and Bayesian extensions) are generally considered state-of-the-art~\mbox{%DIFAUXCMD
\parencite{stamatakis2014, Drummond2007-za, minh2020, Wilgenbusch2003-mu}}\hskip0pt%DIFAUXCMD
. However, approaches based on minimum evolution (ME) have also shown to yield adequate performance~\mbox{%DIFAUXCMD
\parencite{Kuhner1994-cf, Gascuel2006-sr, lefort2015, kumar2000, roch2006}}\hskip0pt%DIFAUXCMD
. The first introductions of the minimum evolution (ME) paradigm~\mbox{%DIFAUXCMD
\parencite{Kidd1971-sk, Rzhetsky1992-qj} }\hskip0pt%DIFAUXCMD
sought to express evolutionary relationships through dissimilarity. They proved that, given unbiased estimates of the true evolutionary distances, the true phylogeny has an expected length shorter than any other possible phylogeny – thereby establishing the principled ME criterion. Currently, the best performing ME approach is that of balanced minimum evolution (BME)~\mbox{%DIFAUXCMD
\parencite{Pauplin2000-vk,Desper2002-uy}}\hskip0pt%DIFAUXCMD
, with }\texttt{\DIFadd{FastME}}\DIFadd{~\mbox{%DIFAUXCMD
\parencite{lefort2015} }\hskip0pt%DIFAUXCMD
being a popular software implementation. Its objective function can be written as:
}\begin{equation}
    \DIFadd{\mathcal{L}(T) = \sum_{i,j}D_{ij}2^{-e_{ij}}
    % \label{eq:bme_objective}
}\end{equation}
\DIFadd{where $D_{ij}$ denotes a distance (e.g., based on molecular sequence data) between two taxa $i$ and $j$ and $e_{ij}$ the number of branches in the path between taxa $i$ and $j$ (the path length~\mbox{%DIFAUXCMD
\parencite{Semple2004-my}}\hskip0pt%DIFAUXCMD
).
This objective can be computed in a numerically stable fashion using the log-sum-exp trick (see Appendix~\ref{append:code} for an example snippet). A widely used approach to estimate the optimal tree greedily~\mbox{%DIFAUXCMD
\parencite{Desper2004-ij, Gascuel2006-sr} }\hskip0pt%DIFAUXCMD
is the neighbour joining (NJ) method~\mbox{%DIFAUXCMD
\parencite{Saitou1987-wg}}\hskip0pt%DIFAUXCMD
. When neighbour joining is based on an additive distance measure, it reconstructs a unique tree, but still performs well with near-additive trees~\mbox{%DIFAUXCMD
\parencite{Atteson1999-jd} }\hskip0pt%DIFAUXCMD
and under small perturbations in the data~\mbox{%DIFAUXCMD
\parencite{Mihaescu2009-es}}\hskip0pt%DIFAUXCMD
. However, despite these highly favourable properties, further heuristic optimisation on a NJ tree using SPR moves have proven to be even more accurate~\mbox{%DIFAUXCMD
\parencite{lefort2015}}\hskip0pt%DIFAUXCMD
. Once a tree topology is found, quadratic algorithms exist for estimating the branch lengths~\mbox{%DIFAUXCMD
\parencite{Mihaescu2008-bo} }\hskip0pt%DIFAUXCMD
as well as efficient approaches for molecular clock dating~\mbox{%DIFAUXCMD
\parencite{To2016-vd}}\hskip0pt%DIFAUXCMD
.
}

\subsubsection*{\DIFadd{Balanced minimum evolution for rooted trees}}

\DIFadd{Inference using BME is always restricted to unrooted trees~\mbox{%DIFAUXCMD
\parencite{Semple2004-my, catanzaro2022} }\hskip0pt%DIFAUXCMD
with rooting chosen after inference through heuristics (e.g., midpoint rooting) or via a molecular clock (e.g., for serially sampled data). However, it is often of interest to find the optimal rooted tree for a set of taxa, as this provides extra biological context (e.g., to represent evolutionary paths).
}

\DIFadd{In an unrooted tree, the BME objective function (Eq.~\ref{eq:bme_objective}) provides an efficient way of calculating the total length of a tree where the branch lengths are the least squares estimators for approximating each $D_{ij}$ with the distance from nodes $i$ to $j$ in the tree. However, this result does not hold in a rooted tree, as the addition of a root changes many of the path lengths. To remedy this, we consider adding a “root taxon” to the tree by joining it to the root node as taxon $n$. If the tree is roughly ultrametric, then we expect
}\begin{equation}
    \DIFadd{D_{ni} \approx D^*  \quad \forall i \neq n
}\end{equation}
\DIFadd{where $D^*$ is the (assumed constant) root-to-taxa distance. Of course, we do not know the sequence of the root but, as we will show, the value of $D^*$ is unimportant — it is instead simply important that it is independent of $i$. Adding this root taxon as a leaf node transforms the tree from being rooted to being unrooted, where standard BME can be used. From this assumption, we prove two lemmas to ensure the framework's validity, showing that the optimal unrooted tree is obtained when the variation in the root-to-taxa distance is sufficiently small (Lemma~\ref{lem:rooted1}), and subsequently that, in all cases, the optimal rooting for an unrooted tree solves a biologically plausible optimisation problem (Lemma~\ref{lem:root_min}).
}

\DIFadd{First, Lemma~\ref{lem:rooted1} shows that, if
}\begin{equation}
    \DIFadd{|D_{ni} - D^*| < \delta \quad \forall i \neq n
}\end{equation}
\DIFadd{then, using $e_{ij}^u$ and $e_{ij}^r$ to denote path lengths in the unrooted tree ($u$) containing taxon $n$ and the rooted tree ($r$) formed by removing taxon $n$,
}\begin{equation}
     \DIFadd{\bigg|\sum_{i=0}^n\sum_{j=0}^nD_{ij}2^{-e^u_{ij}} - \sum_{i=0}^{n-1}\sum_{j=1}^{n-1}D_{ij}2^{-e^r_{ij}} - D^*\bigg| \leq \delta
}\end{equation}
\DIFadd{where $\delta$ denotes a small number. Hence, the difference between the rooted and unrooted objective functions is approximately equal to the constant, $D^*$. Thus, for sufficiently small $\delta$, by the discreteness of tree space, we can see that, if it is unique, the optimal unrooted tree under the }\textit{\DIFadd{rooted}} \DIFadd{objective (using $e_{ij}^r$) will be the same as that under the unrooted objective (using $e_{ij}^u$), when the root taxon is used as an additional leaf.
}

\DIFadd{Subsequently, Lemma~\ref{lem:root_min} shows that, for the correct unrooted tree, the BME-optimal rooting maximizes a simple heuristic (defined in Definition~\ref{def:distance}) for the root-to-tip distance. Equivalently, the optimal rooting ensures that the root is estimated to be the maximal possible distance back in time.
}

\DIFadd{This is not an immediately biologically plausible objective for the root. Indeed, the cornerstone of BME is that we want the tree of }\textit{\DIFadd{minimum}} \DIFadd{length, and it hence seems counter-intuitive to require the root that is the }\textit{\DIFadd{maximum}} \DIFadd{distance backwards in time (though, by Lemma~\ref{lem:root_min}, this does create the minimum length tree). However, the root of our tree must be the point that is furthest backwards in time. In particular, this means that the evolutionary direction needs to be away from the root. By setting our root such that the root-to-tip distance is maximised, we ensure that the root satisfies this constraint.
}

\DIFadd{This method shares a similar motivation with midpoint rooting, which also seeks to maximise a heuristic for root-to-tip distance. However, the heuristic used in midpoint rooting uses only the two taxa which are furthest apart, while our rooting method uses distances from all taxa. Thus, we expect our method to be more robust, particularly as large inter-taxa distances are difficult to estimate, meaning that the additional information used in our heuristic should help to reduce errors. This is evidenced in Fig.~\ref{fig:Songtree}, where midpoint rooting leads to incorrect root placement.
}

\DIFadd{Nonetheless, this property will not hold if the tree is not ultrametric. If taxa evolve at different rates at different times throughout the tree, then the root will be drawn towards taxa with high evolutionary rates. Thus, caution must be used when applying our rooted algorithm to such trees, although the unrooted algorithm will still give a correct unrooted tree. In this case, it may be best to find the optimal unrooted tree topology and then solve the rooting problem for this tree, rather than finding the optimal rooted tree, as the former will reduce the skewing effect of the heterogeneity in evolutionary rates. Because of this, the algorithm introduced in this paper has the flexibility to find the optimal unrooted or rooted tree.
}

\input{fig/fig1}

\DIFaddend \subsubsection*{An ordered bijection to tree space}~Previously, we introduced Phylo2Vec~\DIFdelbegin %DIFDELCMD < \parencite{penn2023}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{penn2023}}\hskip0pt%DIFAUXCMD
}\DIFaddend , a novel bijection between the space of \DIFaddbegin \DIFadd{phylogenetic }\DIFaddend trees and a space of integer vectors. In contrast to other bijections such as \DIFdelbegin \DIFdel{Prüfer codes~}%DIFDELCMD < \parencite{C_Chen2000-ak} %%%
\DIFdel{or }\DIFdelend permutation matchings~\DIFdelbegin %DIFDELCMD < \parencite{diaconis1998}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{diaconis1998}}\hskip0pt%DIFAUXCMD
}\DIFaddend , changes in Phylo2Vec correspond to smooth changes in the tree space, e.g., single changes in a Phylo2Vec vector correspond to a limited set of SPR changes. \DIFaddbegin \DIFadd{On the other hand, Prüfer codes~\mbox{%DIFAUXCMD
\parencite{C_Chen2000-ak} }\hskip0pt%DIFAUXCMD
form a bijection to the space of all $m$-ary trees, meaning that there is no guarantee to sample binary trees from random Prüfer sequences.
}\DIFaddend 

Here, we focus on the notion of \emph{ordered trees} from~\DIFdelbegin %DIFDELCMD < \parencite{penn2023}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{penn2023}}\hskip0pt%DIFAUXCMD
}\DIFaddend , where it is possible to construct a tree from its vector in linear \DIFdelbegin \DIFdel{($\mathcal{O}(n)$) }\DIFdelend time. An ordered tree can be thought of as a birth process, \DIFdelbegin \DIFdel{where }\DIFdelend \DIFaddbegin \DIFadd{such that }\DIFaddend when a birth occurs, the original node continues to live and retains its label, while the new node receives an incremented label. Accordingly, we introduce an equivalent but more intuitive tree construction process for these ordered trees \DIFdelbegin \DIFdel{. }\DIFdelend \DIFaddbegin \DIFadd{(see Fig.~\ref{fig:ltr} for an example). }\DIFaddend We begin with two leaf nodes and two edges labelled 0 and 1. We then append nodes by joining them, \emph{in order}, to edges connecting leaf nodes to the tree. \DIFdelbegin \DIFdel{In Fig.~\ref{fig:ltr}, we first append node 2 to its label edge 0, creating a new internal node and a pair of new edges. The new edge joining node 2 to the tree is labelled as edge 2. We then append node 3 to edge 2, again creating a new internal node and two new edges. }\DIFdelend This tree construction process can be summarised by a single vector $\boldsymbol{v}$, with $v_0 = v_1 = 0$ and, for $m \geq 2$, $v_m$ being the label of the edge to which node $m$ is appended. Each index in $v_m$ is subject to the simple constraint:
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend \begin{align}
\label{eq:disc}
    & v_0 = v_1 = 0 \quad \text{and} \\ 
    & v_m \in \{0,1,...,m-1\} \quad \forall \quad m \geq 2 \nonumber
\end{align}
which is equivalent to the definition of ordered trees in~\DIFdelbegin %DIFDELCMD < \parencite{penn2023}%%%
\DIFdel{. }\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{penn2023}}\hskip0pt%DIFAUXCMD
. Intuitively, a tree is ordered if, starting with a branch connecting the root to taxon 0, the taxa can be added in order of their label by appending a new branch to a }\textit{\DIFadd{terminal}} \DIFadd{branch of the existing tree (i.e. a branch connecting a leaf node to the rest of the tree). Thus, the ordering of the taxa is in some sense ``natural'' for each possible ordered tree.  }\DIFaddend It is proved in \DIFdelbegin \DIFdel{Appendix~\ref{sec:ordered} }\DIFdelend \DIFaddbegin \DIFadd{Lemma~\ref{lem:ltr} }\DIFaddend that for ordered $\boldsymbol{v}$, the algorithm presented above and the more general \DIFaddbegin \DIFadd{Phylo2Vec }\DIFaddend algorithm in~\DIFdelbegin %DIFDELCMD < \parencite{penn2023} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{penn2023} }\hskip0pt%DIFAUXCMD
}\DIFaddend produce equivalent trees.

\DIFdelbegin %DIFDELCMD < \input{fig/fig2}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \DIFadd{Note that, for a fixed integer-taxon labelling, the number of ordered trees is a subset of the number of possible trees. We discuss an efficient method to remedy this problem and explore all tree space in~}\nameref{subsec:queue_shuffle}\DIFadd{.
}\DIFaddend 

\subsubsection*{A continuous representation of a tree}
We introduce \DIFaddbegin \DIFadd{continuous, probabilistic, representation of trees using }\DIFaddend a square matrix $W$ which gives the distribution of a random ordered vector \DIFdelbegin \DIFdel{$\boldsymbol{V}$ }\DIFdelend \DIFaddbegin \DIFadd{$\boldsymbol{v}$ }\DIFaddend with independent entries such that \DIFdelbegin \DIFdel{$W_{ij} = \mathbb{P}(V_i = j)$}\DIFdelend \DIFaddbegin \DIFadd{$W_{ij} = \mathbb{P}(v_i = j)$}\DIFaddend . Given Eq.~\ref{eq:disc}, $W$ is a lower-triangular, stochastic matrix (row sums to 1). \DIFaddbegin \DIFadd{Thus, }\DIFaddend $W$ \DIFdelbegin \DIFdel{is designed to be a continuous representation of a phylogenetic tree, and }\DIFdelend can probabilistically represent any \emph{ordered} phylogenetic tree (a space of \DIFdelbegin \DIFdel{$n!$ }\DIFdelend \DIFaddbegin \DIFadd{$(n-1)!$ }\DIFaddend trees). A simple approach to determining the \DIFdelbegin \DIFdel{best }\DIFdelend \DIFaddbegin \DIFadd{most likely }\DIFaddend single tree from $W$ is to take the column-wise argmax, yielding a single tree $\boldsymbol{v}$.

\DIFaddbegin \subsubsection*{\DIFadd{Gradient-based optimisation using the BME criterion}}
\DIFadd{Using this continuous representation, we can find the optimal ordered tree. Defining $f(\boldsymbol{v})$ to be the BME objective function for the tree generated by an ordered vector $\boldsymbol{v}$, we then create a continuous objective, $F(W)$ by $    F(W) = \mathbb{E}\big[f(\boldsymbol{v})\big]$.
}

\DIFadd{The calculation of $F(W)$ follows our new method of constructing ordered trees from the vector $\boldsymbol{v}$. For a fixed (randomly chosen) tree, we define $e_{ij}^k$ to be the path length between nodes $i$ and $j$ when nodes $0,1,...,k-1$ have been added to the tree (for $i,j < k$). Note that to find the rooted objective function, we initialise with $e_{10}^2 = e_{01}^2 = 2$, while to find the unrooted objective, we initialise with $e_{10}^2 = e_{01}^2 = 1$ (while the Phylo2Vec representation is an inherently rooted representation, this unrooted objective finds the tree length if the root were removed from the random rooted tree with distribution given by $W$). This is because, in a tree where the only leaf nodes are $0$ and $1$, these nodes are a path length of 2 apart if there is also a root (as the root is on this path) while otherwise, they are a path length of 1 apart.
}

\DIFadd{If node $k$ is appended to the edge joining either node $i$ or $j$ to the tree, then $e_{ij}^{k+1} = e_{ij}^k + 1$; otherwise, $e_{ij}^{k+1} = e_{ij}^k$. Similarly, if node $k$ is appended to the edge joining node $i$ to the tree, then $e_{ik}^{k+1} = 2$ and otherwise, if node $k$ is appended to the edge joining node $x$ to the tree, then $e_{ik}^{k+1} = e_{ix}^k + 1$. Thus, using $V_k$ to denote the random value of $v_k$, we can write
}\begin{align}
    &\DIFadd{e^{k+1}_{ij} = e^k_{ij} + G^k_{ij}(V_k) }\\
    &\DIFadd{\Rightarrow e^{n-1}_{ij} = \sum_{k=2}^{n-2}G^k_{ij}(V_k) + e^2_{ij}
}\end{align}
\DIFadd{for some functions $G^k_{ij}$ which are derived explicitly in Lemma~\ref{lem:cont_obj}. Importantly, each term in the sum is independent, and hence, in Lemma \ref{lem:cont_obj}, a closed iterative system for the quantities $E_{ij}^{k} = \mathbb{E}(2^{-e_{ij}^k})$ can be calculated for $i<j$ as
}\begin{equation}
        \DIFadd{E_{ij}^{k+1} = \left\{ \begin{matrix}
            E^{k}_{ij} \bigg[1 - \frac{1}{2}(W_{ki} + W_{kj})\bigg] & \text{if $i < j < k$}\\
              \bigg[\frac{1}{2}\sum_{x\neq i}E_{ix}^kW_{kx}\bigg] + \frac{1}{4}W_{ki} & \text{if $i < k$}
        \end{matrix}\right.
    }\end{equation}
    \DIFadd{with the remaining values for $i > j$ following by symmetry.
}

\DIFadd{The objective function is a polynomial function of the entries of $W$ and is linear in each fixed entry (that is, the diagonal entries of $\nabla^2 F$ are zero). Thus, by Lemma~\ref{lem:discrete}, there is always a minimum at a “discrete tree'' (that is, at a matrix $W$ where for each row, one value is 1 and all the others are 0). Moreover, this simple form makes it easy to differentiate $F$ analytically, numerically or automatically. Using state-of-the-art automatic differentiation~\mbox{%DIFAUXCMD
\parencite{jax2018github}}\hskip0pt%DIFAUXCMD
, gradient descent can be used to efficiently minimise $F$ and find the optimal }\textit{\DIFadd{ordered}} \DIFadd{tree. 
}

\DIFadd{There may also be minima at non-discrete trees if multiple trees share the same, optimal, objective value. In our rooted optimisation, this is highly unlikely (as two topologically different trees having equal objectives places a dimension 1 condition on the distance matrix $D$, meaning the set of distance matrices for which this happens has measure 0 in the set of possible distance matrices), but when we use our unrooted algorithm, this will occur. This is because, as discussed in \mbox{%DIFAUXCMD
\parencite{penn2023}}\hskip0pt%DIFAUXCMD
, there are $n-1$ Phylo2Vec vectors which, when the root is removed, give the same unrooted tree. Thus, if multiple rooted vectors giving the same unrooted tree $\mathcal{U}$ are in the same space of ordered trees, then, if $\mathcal{U}$ is the optimal tree under this ordering, the algorithm may converge to a non-discrete $W$. In this case, taking the argmax safely recovers an optimal rooted tree as, by Lemma~\ref{lem:discrete}, all possible trees according to $W$ will have the optimal objective value.
}

\DIFadd{The tree-space induced by our continuous objective function will have local minima whenever changing any single entry of the vector $\boldsymbol{v}$ causes the objective function to increase. As the Hamming distance between vectors $\boldsymbol{u}$ and $\boldsymbol{v}$ is comparable to SPR distance~\mbox{%DIFAUXCMD
\parencite{penn2023}}\hskip0pt%DIFAUXCMD
, we therefore expect that the discrete subset of our continuous tree-space will be similar in structure to the space induced by SPR moves. However, by starting from a uniformly distributed tree, where all possible ordered trees contribute to the objective, we expect that our algorithm is better able to pick up the ``signal'' from the true optimum, and avoid moving towards suboptimal local minima.
}

\DIFadd{A Python-like algorithm to compute $ \mathbb{E}(2^{-e})$ is shown in Algorithm~\ref{algo:get_edges_exp}. To find the $E^m_{ij}$ terms, there are $\mathcal{O}(m)$ steps of $\mathcal{O}(m)$ (finding the $E_{m-1, j}^m$ terms) and $\mathcal{O}(m^2)$ steps of $\mathcal{O}(1)$ (finding the other $E_{ij}^m$ terms). There are $\mathcal{O}(n)$ values of $m$ that need to be considered, and hence this system can be solved in $\mathcal{O}(n^3)$ time.
}

\begin{algorithm}
\caption{\DIFadd{Compute $E := \mathbb{E}(2^{-e})$ }}  \label{algo:get_edges_exp}
\begin{algorithmic}[1]
\Require \DIFadd{$n$ }\Comment{fixed number of taxa}
\Require \DIFadd{$W$ }\Comment{stochastic input matrix\parencite{penn2023}}
\State \DIFadd{$E = \text{{zeros}}((n, n))$
}\For{$i \gets 1$ \text{{ to }} $n - 1$}
    \State \DIFadd{$E^* = \text{{zeros}}((n, n))$
    }\For{$k \gets 0$ \text{{ to }} $i - 1$}
        \For{$j \gets 0$ \text{{ to }} $k - 1$}
            \State \DIFadd{$E^*_{[k,j]} = E_{[k,j]} (1 - \frac{1}{2} (W_{[i-1,j]} + W_{[i-1,k]}))$
        }\EndFor
        \State \DIFadd{$E^*_{[i,k]}= \sum_{l=0}^{i-1} \frac{1}{2} E_{[l,k]} W_{[i-1,l]} + \frac{1}{4}  W_{[i-1,k]}$
    }\EndFor
    \State \DIFadd{$E = E^* + E^{*T}$
}\EndFor
\State \DIFadd{\text{{Return }} $E$
}\end{algorithmic}
\end{algorithm}

\subsubsection*{\DIFadd{Orderings}}
\DIFadd{The continuous objective function is only defined for ordered trees, which, for a given labelling of the nodes, is a subset of the whole tree space. Thus, we define the concept of an }\textit{\DIFadd{ordering}} \DIFadd{of the nodes, whereby changing the ordering allows the full space of trees to be explored.
}

\begin{definition}
   \textbf{\DIFadd{Ordering:}} \DIFadd{Suppose that the nodes correspond to taxa with names $N_0,N_1,...N_{n-1}$. We then define an }\textit{\DIFadd{ordering}} \DIFadd{of the nodes to be a permutation, $\sigma$ of the set $\{0,...,n-1\}$ such that the node with name $N_i$ is processed as node $\sigma(i)$ by the Phylo2Vec algorithm. It is necessary that the associated Phylo2Vec vector $\boldsymbol{v}(\sigma)$ is ordered.
}\end{definition}
\DIFadd{Note that we use the phrase “node $x$'' to mean “the node with name $N_x$'' and will always be explicit if we refer to a node by its label.
}

\DIFadd{Given a tree, it is possible to generate a possible ordering of the nodes, $\sigma$, as well as the associated vector $\boldsymbol{v}(\sigma)$. We will do this by labelling the tree as follows, again distinguishing between the leaf node names $N_i$ and their labels (which we will call $l(i)$).
}

\DIFadd{Consider labelling the root node as 0. Then, label the children of this node as $0$ and $1$. One can continue this process inductively, choosing a node, labelled $x$, with unlabelled children and then labelling its children as $x$ and $y$, where $y$ is the smallest unused label. This process terminates when every node has been labelled. As discussed above, suppose that the label of the leaf node with name $N_i$ is $l(i)$. Then, Lemmas \ref{lem:ordering_1}, \ref{lem:ordering_2} and \ref{lem:ordering_3} show that $l$ is a possible ordering of the tree, and provide a method for calculated the associated ordered Phylo2Vec vector $\boldsymbol{v}(l)$.
}

\DIFadd{Given a tree, one can use the previous labelling algorithm to show that there are at least $2^{n-1}$ possible orderings for the tree (as the children of each node can be labelled in either order). The exact number depends on the choice of which internal node is processed at each step (and so, a “flat'' tree where the leaves have a low generation has more possible orderings than a “ladder'' tree where each leaf has a distinct generation). However, in general, it will be substantially larger than $2^{n-1}$ (we conjecture that for flat trees, it may be factorial in size) and hence there are numerous possibilities which will allow for a global minimum of the objective to be found.
}\DIFaddend \subsubsection*{Queue Shuffle: changing orderings to explore all the tree space}
\DIFaddbegin \label{subsec:queue_shuffle}
\DIFaddend The number of ordered trees \DIFaddbegin \DIFadd{(different from ranked trees~\mbox{%DIFAUXCMD
\parencite{Collienne2021-eg}}\hskip0pt%DIFAUXCMD
), $(n-1)!$}\DIFaddend , \DIFdelbegin \DIFdel{$n!$, }\DIFdelend is substantially smaller than the possible number of trees, $(2n-3)!!$ (\DIFdelbegin \DIFdel{although }\DIFdelend \DIFaddbegin \DIFadd{albeit }\DIFaddend with a comparable growth pattern in $n$), and hence, \DIFaddbegin \DIFadd{while }\DIFaddend the optimal ordered tree \DIFdelbegin \DIFdel{is likely to be close to , but not }\DIFdelend \DIFaddbegin \DIFadd{will be closer to the true tree than a very large proportion of trees, it is very unlikely to be }\DIFaddend exactly equal to \DIFdelbegin \DIFdel{, the true optimal }\DIFdelend \DIFaddbegin \DIFadd{the true }\DIFaddend tree. 

To fully explore tree space, \DIFdelbegin \DIFdel{we randomly change }\DIFdelend \DIFaddbegin \DIFadd{one must shuffle }\DIFaddend the labels of the leaf nodes in the optimal ordered tree\DIFdelbegin \DIFdel{using a }\DIFdelend \DIFaddbegin \DIFadd{. Simply choosing a uniformly random permutation will lead to extremely inefficient optimisation, as each tree is only possible in approximately $1/2^{n}$ of the possible orderings. Instead, we use the topology of the optimal tree to inform our choice of permutation through a }\DIFaddend novel approach we call the \textit{Queue Shuffle}\DIFdelbegin \DIFdel{(full details in Appendix~\ref{sec:queue_shuffle}).
Shuffling amounts to choosing a permutation $\sigma$ on $\{0,1...,n-1\}$ such that the leaf with name $N_i$ now has label $\sigma(i)$.
We call this an }\textit{\DIFdel{ordering}} %DIFAUXCMD
\DIFdel{of the leaf nodes .
}\DIFdelend \DIFaddbegin \DIFadd{. This ensures that the previous optimal tree can be written as an ordered tree in the new ordering, while also ensuring a smooth and efficient path through the space of orderings.
}\DIFaddend 

\DIFdelbegin \DIFdel{Each different ordering changes the explorable space of ordered trees}\DIFdelend \DIFaddbegin \DIFadd{The Queue Shuffle is motivated by the labelling procedure discussed in the previous section, but ensures that the set of internal nodes with a given generation (that is, a given distance from the root) are processed consecutively. That is, we begin by processing all nodes with generation 0 (i.e., the root), then all internal nodes with generation 1, then all internal nodes with generation 2, and continue in this fashion until all internal nodes have been processed.
}\\
\\
\noindent
\DIFadd{Algorithmically, this can be achieved by a “queue'' of internal nodes to be processed. When an internal node is processed, any of its children that are also internal nodes are added to the back of this queue}\DIFaddend . Thus, \DIFdelbegin \DIFdel{once an ordering is chosen, one can re-optimise an objective function $F(W)$ in this new space of ordered trees (note that the previous optimal tree is still in this space and so, provided it finds the true optimal ordered tree, it will have an objective value no worse than the previous tree). This process is then repeated, re-ordering the tree and re-optimising in the new space , until the best found tree does not change for a certain }\DIFdelend \DIFaddbegin \DIFadd{the queue is always in ascending order of generation, and it is simple to show that this ensures that nodes are processed in non-decreasing order of generation. 
}\\
\\
\noindent
\DIFadd{A crucial feature of this queue is that the child given the same label as its parent is placed }\textit{\DIFadd{ahead}} \DIFadd{of the other child in the queue. This ensures that one can, in some way, control the order of processing by choosing the labelling of the children of each node. Moreover, it is vital for the theoretical result presented in the following section. 
}\\
\\
\noindent
\DIFadd{To add randomness into the labelling procedure, every time an internal node is processed, we randomly choose which child is given the label of their parent, and which child is given the next available label. This provides $2^{n-1}$ possible orderings for each tree. This stochasticity is helpful in ensuring that the algorithm does not get stuck – as discussed in the subsequent section, it ensures that a large class of similar trees will be considered after a few ordering proposals.
}

\DIFadd{An algorithmic description of the Queue Shuffle is provided in Algorithm \ref{algo:qs}.
}

\begin{algorithm}
\caption{\DIFadd{The Queue Shuffle }}  \label{algo:qs}
\begin{algorithmic}[1]
\Require \DIFadd{$\mathcal{T}$ }\Comment{Current Tree}
\Require \DIFadd{$\mathcal{N} = \{\nu_0,\nu_1,...\}$ }\Comment{set of all non-root nodes}
\State \DIFadd{$Q = [\nu_0,\nu_1]$ }\Comment{"queue" of nodes to process}
\State \DIFadd{$L = \{\nu_0 : 0, \nu_1 : 1\}$ }\Comment{node:label mapping}
\State \DIFadd{$l_{\text{next}} = 2$}\Comment{next available label}
\State \DIFadd{$P = []$ }\Comment{processed nodes}
\While{$Q \neq []$}
\State \DIFadd{$\nu = Q[0]$ }\Comment{node to process}
\State \DIFadd{Q = Q}[\DIFadd{1:}] \Comment{$\nu$ will be processed}
\State \DIFadd{$\text{append}(P,\nu)$ }\Comment{$\nu$ will be processed}
\If{$\text{isLeaf}(\nu)$}
\State \textbf{\DIFadd{continue}} \Comment{move to next node}
\EndIf
\State \DIFadd{$a,b = \text{randChildren}(\nu)$ }\Comment{get \textbf{randomly ordered} children of $\nu$}
\State \DIFadd{$L[a] = L[\nu]$ }\Comment{label $a$ with $\nu$'s label}
\State \DIFadd{$L[b] =  l_{\text{next}}$ }\Comment{give $b$ next available label}
\State  \DIFadd{$l_{\text{next}} =  l_{\text{next}} +1$
}\State \DIFadd{append($Q,a$) }\Comment{add $a$ to the queue}
\State \DIFadd{append$(Q,b)$ }\Comment{add $b$ to the queue}
\EndWhile
\State \DIFadd{\text{{Return }} $L$ }\Comment{Ordering determined by values of $L$ for leaf nodes}
\end{algorithmic}
\end{algorithm}


\subsubsection*{\DIFadd{GradME}}
\DIFadd{The Queue Shuffle completes our optimisation algorithm. We iteratively find the best ordered tree according to the current ordering and then use Queue Shuffle to change ordering, changing the space of explorable trees. The algorithm terminates when the optimal tree has not been improved upon for a fixed }\DIFaddend number of iterations \DIFdelbegin \DIFdel{. In practice, only ten to twenty }\DIFdelend \DIFaddbegin \DIFadd{(note that, by construction, the previous optimal tree will always be in the new space of ordered trees). In the examples presented in this paper, only tens }\DIFaddend iterations are needed from some random starting order, and less if a sensible \DIFdelbegin \DIFdel{start }\DIFdelend \DIFaddbegin \DIFadd{starting ordering }\DIFaddend (such as from a neighbour joining tree) is used.

\DIFaddbegin \DIFadd{We refer the resulting system, combining the continuous tree representation, Queue Shuffle reordering, and the gradient-based optimisation framework using BME, as }\textsb{\DIFadd{GradME}}\DIFadd{. 
}


\subsubsection*{\DIFadd{Why does Queue Shuffle work?}}
\DIFaddend A given tree is in the space of ordered trees for at least $2^{n-1}$ orderings. This means that we do not need to find a single optimal ordering, but have exponentially many which will return the true optimal tree. Very loosely considered, being able to explore $n!$ tree space reliably and efficiently with continuous optimisation, Queue Shuffle reduces the inferential task to one that is exponential.

\DIFdelbegin \subsubsection*{\DIFdel{Why does Queue Shuffle work?}}
%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{While }\DIFdelend \DIFaddbegin \DIFadd{However, while }\DIFaddend the number of optimal orderings grows exponentially, their proportion tends quickly to zero as $n$ grows. It is therefore, perhaps, surprising that we are able to find an optimal ordering so quickly from merely tens of shuffles. The proportion of optimal orderings (approximately the ratio of ordered trees to total trees, $\frac{(n-1)!}{(2n-3)!!}$\DIFdelbegin \DIFdel{) }\DIFdelend \DIFaddbegin \DIFadd{, }\DIFaddend ranges from $8\times 10^{-4}$ in our smallest dataset (14 taxa) to $6\times 10^{-29}$ in the largest (99 taxa\DIFaddbegin \DIFadd{; see Table~\ref{tab:data}}\DIFaddend ).

\DIFdelbegin \DIFdel{However, our algorithmis able to find these optimal orderingsbecause the Queue Shuffle does not choose the new ordering uniformly over the space of orderings (which is $n!$ large).
Instead, the distribution depends on the structure of the tree and therefore facilitates sensible proposals. For example}\DIFdelend \DIFaddbegin \DIFadd{This efficiency comes from the topology-dependence of the Queue Shuffle algorithm, which allows us to plot a relatively ``smooth'' path through the space of possible orderings. That is, the majority of trees in the new ordered space will have similar properties to the previous optimal tree and so, unless the previous tree was a local minimum of the objective, it is likely that one of these ``close'' trees will have a lower objective value.
}

\DIFadd{Lemma~\ref{lem:asym} shows that the expected distance from the root grows harmonically as the label increases. For large trees, the node with label $n-1$ has an expected distance from the root of approximately twice the expected distance from the root of the node label $0$. This property is noticeable even for small trees – if $n = 10$, then the ratio of the expected distance to the root of node 9 and node 0 is approximately $1.65$. Thus}\DIFaddend , nodes which are close to the root \DIFdelbegin \DIFdel{are always given low labels, meaning that they }\DIFdelend \DIFaddbegin \DIFadd{in the current optimum, }\DIFaddend will also be \DIFdelbegin \DIFdel{close }\DIFdelend \DIFaddbegin \DIFadd{closer on average }\DIFaddend to the root in \DIFdelbegin \DIFdel{a high proportion of the }\DIFdelend \DIFaddbegin \DIFadd{the new space of ordered trees. In essence, this means that “fewer slots are wasted'' in the new ordered space – that is, there are fewer }\DIFaddend trees in the new space of ordered trees \DIFdelbegin \DIFdel{(cf. Appendix~\ref{sec:queue_shuffle}).
}\DIFdelend \DIFaddbegin \DIFadd{which are topologically far from the previous optimum (a tree that, after the first few iterations, is likely to be far closer to the true optimum than a randomly-chosen tree) and hence, more trees which are reasonable candidates for having lower objective values.
}\DIFaddend 

\DIFdelbegin \DIFdel{When a good tree is found in some ordered space, it is reasonable to expect a better treewill retain similarities with the good tree, and the Queue Shuffle allows for these trees to be explored.
Theorem 1 in Appendix~\ref{sec:queue_shuffle} formalises the }\textit{\DIFdel{swapping property}} %DIFAUXCMD
\DIFdel{of the }\DIFdelend \DIFaddbegin \DIFadd{Lemma~\ref{fig:swap} proves another example of the smoothness in transitions induced by the }\DIFaddend Queue Shuffle, \DIFdelbegin \DIFdel{illustrated in Fig. ~\ref{fig:swap}. Given any pair of subtrees which are connected to the tree by two }\DIFdelend \DIFaddbegin \DIFadd{based on nearest neighbour interchange (NNI) moves. An NNI move considers the four subtrees attached to two non-root }\DIFaddend nodes that share an edge \DIFdelbegin \DIFdel{, the swapping property states that, with at least probability $\frac{1}{4}$, a tree that is identical to the previous optimum, with the exception that these two subtrees are swapped, }\DIFdelend \DIFaddbegin \DIFadd{and swaps two of these subtrees. Lemma~\ref{fig:swap} shows that, starting from a tree $\mathcal{T}$, any tree which is one NNI move away from $\mathcal{T}$ }\DIFaddend will be in the new space of ordered trees \DIFdelbegin \DIFdel{. }\DIFdelend \DIFaddbegin \DIFadd{with probability at least $\frac{1}{4}$. 
}

\DIFaddend This ensures that this new space  contains many sensible proposal trees. \DIFdelbegin \DIFdel{Moreover, the fact }\DIFdelend \DIFaddbegin \DIFadd{Perhaps the most surprising aspect of this theorem is }\DIFaddend that this probability is bounded below\DIFdelbegin \DIFdel{by a fixed constant, independent of the size of the phylogeny, is a surprising, and powerful property: it means that there is a sense of continuity when moving between ordered tree spaces}\DIFdelend \DIFaddbegin \DIFadd{, independently of the topology. Thus, with high probability, the optimal tree will only remain the same for more than a few iterations if large sets of similar trees yield lower objective values than the current optimum}\DIFaddend . 

\DIFdelbegin \subsubsection*{\DIFdel{Balanced minimum evolution}}%DIFAUXCMD
\DIFdel{~Popular objective functions for inferring the best treegiven some data include maximum parsimony~}%DIFDELCMD < \parencite{Fitch1967-dr}%%%
\DIFdel{, maximum likelihood~}%DIFDELCMD < \parencite{felsenstein1983} %%%
\DIFdel{and minimum evolution~}%DIFDELCMD < \parencite{Saitou1987-wg}%%%
\DIFdel{. Of these three, only maximum likelihood and minimum evolution are provably statistically consistent~}%DIFDELCMD < \parencite{Desper2004-ij,felsenstein2004} %%%
\DIFdel{(maximum parsimony can be inconsistent under certain conditions~}%DIFDELCMD < \parencite{Felsenstein1978-jt}%%%
\DIFdel{) . For small to moderate sized phylogenies, maximum likelihood (and Bayesian extensions) is generally considered state-of-the-art~}%DIFDELCMD < \parencite{stamatakis2014, Drummond2007-za, minh2020, Wilgenbusch2003-mu}%%%
\DIFdel{, but approaches based on minimum evolution have also consistently shown to yield comparable performance~}%DIFDELCMD < \parencite{Kuhner1994-cf, Gascuel2006-sr, lefort2015, kumar2000, roch2006}%%%
\DIFdel{.
The first introductions of the minimum evolution paradigm~}%DIFDELCMD < \parencite{Kidd1971-sk, Rzhetsky1992-qj} %%%
\DIFdel{sought to express evolutionary relationships through dissimilarity. They proved that, given unbiased estimates of the true evolutionary distances, the true phylogeny has an expected length shorter than any other possible phylogeny – thereby establishing a principled objective criterion. Currently, the best performing minimum evolution approach is that of balanced minimum evolution (BME)~}%DIFDELCMD < \parencite{Pauplin2000-vk,Desper2002-uy} %%%
\DIFdel{(with the widely used software implementation }\texttt{\DIFdel{FastME}}%DIFAUXCMD
\DIFdel{~ }%DIFDELCMD < \parencite{lefort2015}%%%
\DIFdel{). Given $D_{ij}$, the distance between two taxa $i$,$j$, (where this distance could be based on morphology, molecular sequences etc.) and $e_{ij}$, the number of branches in the path between taxa $i$ and $j$ (the path length ~}%DIFDELCMD < \parencite{Semple2004-my}%%%
\DIFdel{), the objective function for a given tree $T$ is:
}\begin{displaymath}
    \DIFdel{\mathcal{L}(T) = \sum_{i,j}D_{ij}2^{-e_{ij}}
    \label{eq:bme_objective}
}\end{displaymath}%DIFAUXCMD
\DIFdel{This objective can be computed in a numerically stable fashion using the log-sum-exp trick. A widely used approach to estimate the optimal treegreedily~}%DIFDELCMD < \parencite{Desper2004-ij, Gascuel2006-sr} %%%
\DIFdel{is the neighbour joining method~}%DIFDELCMD < \parencite{Saitou1987-wg}%%%
\DIFdel{. When neighbour joining is based on an additive distance measure, it reconstructs a unique tree, but still performs well with near-additive trees~}%DIFDELCMD < \parencite{Atteson1999-jd} %%%
\DIFdel{and under small perturbations in the data~}%DIFDELCMD < \parencite{Mihaescu2009-es}%%%
\DIFdel{. However, despite these highly favourable properties, further heuristic optimisation on a neighbour joining tree utilising subtree-prune and regrafting have proven to be even more accurate~}%DIFDELCMD < \parencite{lefort2015}%%%
\DIFdel{. Once a tree topology is found, quadratic algorithms exist for estimating the branch lengths~}%DIFDELCMD < \parencite{Mihaescu2008-bo} %%%
\DIFdel{as well as efficient approaches for molecular clock dating~}%DIFDELCMD < \parencite{To2016-vd}%%%
\DIFdelend \DIFaddbegin \DIFadd{That being said, the Queue Shuffle does not guarantee that the global minimum will be found, even if the gradient-based algorithm for optimising $F(W)$ always converges to the optimal tree}\DIFaddend . \DIFaddbegin \DIFadd{If a tree is “far'' from the nearest tree with a better objective value, then it may take a very large number of shuffles (or, indeed, it may be impossible) to find a better tree. However, while the only theoretical guarantee is that Lemma~\ref{fig:swap} shows it will quickly find better trees that can be formed by NNI, we expect that stronger conditions hold on its ability to “escape'' from local minima.
}\DIFaddend 

\DIFdelbegin \subsubsection*{\DIFdel{Balanced minimum evolution for rooted trees}}
%DIFAUXCMD
\DIFdelend \DIFaddbegin \input{tab/table1}
\DIFaddend 

\DIFdelbegin \DIFdel{Inference using BME is almost always restricted to unrooted trees~}%DIFDELCMD < \parencite{Semple2004-my} %%%
\DIFdel{with rooting chosen after inference through heuristics (e.g., midpoint rooting) or via a molecular clock (e.g., for serially sampled data) . However, it is often of interest to find the optimal rooted tree for }\DIFdelend \DIFaddbegin \subsubsection*{\DIFadd{Computational complexity}}

\DIFadd{The computational complexity for all distance-based algorithms requires an upfront computational cost of $\mathcal{O}(n^2)$ to compute the distance matrix. We will disregard this cost from subsequent comparisons. The standard neighbour-joining algorithm~\mbox{%DIFAUXCMD
\parencite{saitou1987} }\hskip0pt%DIFAUXCMD
has an overall computational complexity of $\mathcal{O}(n^3)$. FastME has a computational complexity of $\mathcal{O}(k n^2 _ \text{Diam}(T))$ (where Diam$(T)$ is the maximum path length in }\DIFaddend a \DIFdelbegin \DIFdel{set of taxa, as this provides extra biological context. }%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{In an unrooted tree, the BME objective function (Eq.~\ref{eq:bme_objective}) provides an efficient way of calculating the total length of a tree where the branch lengths are the least squares estimators for approximating each $D_{ij}$ with the distance from nodes $i$ to $j$ in the tree. However, this result does not hold in a rooted tree, as the addition of }\DIFdelend \DIFaddbegin \DIFadd{tree, which is generally much smaller than $n$) for $k$ iterations where $k<n$ when $n$ is large. When fully discrete, our algorithm also has same complexity but with added mechanisms for escaping optima via Queue Shuffle. Therefore, }\DIFaddend a \DIFdelbegin \DIFdel{root changes some path lengths}\DIFdelend \DIFaddbegin \DIFadd{discrete setting is as computationally efficient as FastME (see Appendix~\ref{append:est} for details)}\DIFaddend . 

\DIFdelbegin \DIFdel{To remedy this, we consider adding a hypothetical and very distant, root (as node $n$) into the tree and finding the optimal unrooted tree with these $n+1$ taxa. We can create a rooted tree by removing node $n$ and, as we know that node $n$ evolved first, this will be the root of the original $n$ taxa. Moreover, we show in Appendix~\ref{sec:bme_rooted} that, to leading order, the BME objective applied to this rooted tree differs only by a constant from the BME objective applied to the unrooted tree with $n+1$ taxa. Thus, BME provides a sensible method for finding the optimal rooted tree and can be sensibly applied directly to a rooted topology. However, as discussed in detail in Appendix~\ref{sec:bme_rooted}, it will struggle to find the correct root of trees that are not ultrametric as the root will be drawn towards taxa that are more distant from the root.
}%DIFDELCMD < 

%DIFDELCMD < %%%
\subsubsection*{\DIFdel{Gradient-based optimisation using the BME criterion}}
%DIFAUXCMD
\DIFdel{Defining $f(\boldsymbol{v})$ to be the BME objective functionfor the tree generated by $\boldsymbol{v}$, we then create a continuous objective, $F(W)$ by $    F(W) = \mathbb{E}\bigg[f(\boldsymbol{V})\bigg]$. We present in Appendix~\ref{sec:cont_edge} a novel method for calculating this objective function in cubic time (}\DIFdelend \DIFaddbegin \DIFadd{Computing the expectation in Algorithm~\ref{algo:get_edges_exp} has complexity }\DIFaddend $\mathcal{O}(n^3)$\DIFdelbegin \DIFdel{; where $n$ is the number of taxa). We can perform inference on this objective for both rooted and unrooted trees.
}\DIFdelend \DIFaddbegin \DIFadd{. A single gradient evaluation (that is, calculating $\frac{\partial F}{\partial W_{ij}}$ for some $i$ and $j$) is also $\mathcal{O}(n^3)$ and therefore computing the full Jacobian is $\mathcal{O}(n^5)$. Our Queue Shuffle algorithm runs in $\mathcal{O}(n)$. Therefore, our optimisation for $k$ steps and $l$ shuffles yields a complexity of $\mathcal{O}(kln^5)$. The size of $l$ is dependent on the choice of gradient optimiser, and the size of $k$ varies if a sensible ordering is initialised. 
}\DIFaddend 

\DIFdelbegin \DIFdel{An important property of our continuous objective function is that there is always a minimum at a “discrete tree'' – that is, at a matrix }\DIFdelend \DIFaddbegin \DIFadd{Thus, the computational complexity of GradME is substantially higher than that of FastME and closer to that of FITCH~\mbox{%DIFAUXCMD
\parencite{felsenstein1997alternating}}\hskip0pt%DIFAUXCMD
. This is due to the far greater mathematical complexity of the continuous objective function, $F(W)$. As it is an expectation over all possible ordered trees, the explicit formula for $F(W)$ is a polynomial in }\DIFaddend $W$ \DIFdelbegin \DIFdel{where for each row, one value is 1 and all the others are 0 (e.g., see Fig. ~\ref{fig:big_jump}). Moreover, the objective function is a polynomial function of the entries of $W$ and is linear in each fixed entry (that is, the diagonal entries of $\nabla^2 F$ are zero), making it easy to differentiate analytically, numerically or automatically. Using state-of-the-art automatic differentiation~}%DIFDELCMD < \parencite{jax2018github}%%%
\DIFdel{, gradient descent can be used to efficiently minimize $F$ and find the optimal }\textit{\DIFdel{ordered}} %DIFAUXCMD
\DIFdel{tree}\DIFdelend \DIFaddbegin \DIFadd{with $(n-1)!$ different terms. Intuitively, the continuous space always considers a path between any two trees, something that becomes impossible with discrete settings. Thus, being able to compute it in polynomial time is a vast improvement on a naive approach, although it is still considerably less than the innovative FastME greedy approach. More savings should be possible, we hope to make further efficiency gains in future work}\DIFaddend . 

\DIFdelbegin \DIFdel{We refer the resulting system, combining the continuous tree representation, Queue Shuffle reordering, and the gradient-based optimisation framework using BME, as }\textsb{\DIFdel{GradME}}%DIFAUXCMD
\DIFdel{.
}%DIFDELCMD < 

%DIFDELCMD < \input{tab/table1}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend \subsubsection*{Evaluation} We evaluate GradME on a diverse corpus of 14 empirical molecular sequence datasets (Table~\ref{tab:data}). The first 11 are commonly used to assess phylogenetic inference performance~\DIFdelbegin %DIFDELCMD < \parencite{Whidden2015-jn}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Whidden2015-jn}}\hskip0pt%DIFAUXCMD
}\DIFaddend , whereas the last three were used to assess inference on rooted trees. For each dataset, we start from a random tree and optimise the $W$ matrix to a tolerance of 1e-10 using gradient descent with Adafactor~\DIFdelbegin %DIFDELCMD < \parencite{shazeer2018} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{shazeer2018} }\hskip0pt%DIFAUXCMD
}\DIFaddend optimisation. The distance matrix $D$ is computed using the \DIFdelbegin \DIFdel{F81 }\DIFdelend \DIFaddbegin \DIFadd{GTR+$\Gamma$ }\DIFaddend substitution model for DNA \DIFdelbegin \DIFdel{~}%DIFDELCMD < \parencite{felsenstein1981}%%%
\DIFdel{, and LG~}%DIFDELCMD < \parencite{Le2008-ut} %%%
\DIFdelend \DIFaddbegin \DIFadd{and an LG model~\mbox{%DIFAUXCMD
\parencite{Le2008-ut} }\hskip0pt%DIFAUXCMD
}\DIFaddend for amino acids. \DIFaddbegin \DIFadd{Substitution model parameters for the GTR+$\Gamma$ are also estimated using gradient descent with Adafactor using a pairwise maximum likelihood approach~\mbox{%DIFAUXCMD
\parencite{yang2006}}\hskip0pt%DIFAUXCMD
. }\DIFaddend Jukes-Cantor~\DIFdelbegin %DIFDELCMD < \parencite{jukes1969} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{jukes1969}}\hskip0pt%DIFAUXCMD
, F81~\mbox{%DIFAUXCMD
\parencite{felsenstein1981} }\hskip0pt%DIFAUXCMD
}\DIFaddend and TN93~\DIFdelbegin %DIFDELCMD < \parencite{tamura1993} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{tamura1993} }\hskip0pt%DIFAUXCMD
}\DIFaddend models were also \DIFdelbegin \DIFdel{considered }\DIFdelend \DIFaddbegin \DIFadd{tested }\DIFaddend for DNA, while stochastic gradient descent (SGD), RMSprop~\DIFdelbegin %DIFDELCMD < \parencite{tieleman2012}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{tieleman2012}}\hskip0pt%DIFAUXCMD
}\DIFaddend , and AdamW~\DIFdelbegin %DIFDELCMD < \parencite{Kingma2014-ow, loshchilov2018} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Kingma2014-ow, loshchilov2018} }\hskip0pt%DIFAUXCMD
}\DIFaddend were also considered for optimisation (see Fig.~\ref{fig:convergence_analysis}). \DIFdelbegin \DIFdel{As a baseline, we compute the mean BME loss over 50 random uniform trees, sampled using Phylo2Vec~}%DIFDELCMD < \parencite{penn2023}%%%
\DIFdel{. }\DIFdelend To fairly assess the performance of GradME, we compare our framework to two well-established distance-based methods: \texttt{BioNJ}~\DIFdelbegin %DIFDELCMD < \parencite{gascuel1997}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{gascuel1997}}\hskip0pt%DIFAUXCMD
}\DIFaddend , based on the neighbour joining algorithm~\DIFdelbegin %DIFDELCMD < \parencite{saitou1987}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{saitou1987}}\hskip0pt%DIFAUXCMD
}\DIFaddend , and \texttt{FastME}~\DIFdelbegin %DIFDELCMD < \parencite{lefort2015}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{lefort2015}}\hskip0pt%DIFAUXCMD
}\DIFaddend , based on balanced minimum evolution.

\vspace{-1em}

\subsubsection*{Implementation} Implementation of the BME criterion and \DIFdelbegin \DIFdel{of }\DIFdelend the optimisation framework was written in Python using \texttt{Jax}~\DIFdelbegin %DIFDELCMD < \parencite{jax2018github} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{jax2018github} }\hskip0pt%DIFAUXCMD
}\DIFaddend and \texttt{Optax}~\DIFdelbegin %DIFDELCMD < \parencite{deepmind2020}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{deepmind2020}}\hskip0pt%DIFAUXCMD
}\DIFaddend . Optimisation was performed on a Xeon 2.30GHz (CPU; Intel Corporation) or on a single GeForce GTX 1080 (GPU; Nvidia Corporation). Evaluation of the \texttt{BioNJ}~\DIFdelbegin %DIFDELCMD < \parencite{gascuel1997} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{gascuel1997} }\hskip0pt%DIFAUXCMD
}\DIFaddend and \texttt{FastME}~\DIFdelbegin %DIFDELCMD < \parencite{lefort2015} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{lefort2015} }\hskip0pt%DIFAUXCMD
}\DIFaddend methods was performed via the R package \texttt{ape}~\DIFdelbegin %DIFDELCMD < \parencite{paradis2004} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{paradis2004} }\hskip0pt%DIFAUXCMD
}\DIFaddend using \texttt{rpy2}~\DIFdelbegin %DIFDELCMD < \parencite{rpy2}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{rpy2}}\hskip0pt%DIFAUXCMD
}\DIFaddend . Tree manipulation and visualisation scripts were written using \texttt{ete3}~\DIFdelbegin %DIFDELCMD < \parencite{huerta2016} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{huerta2016} }\hskip0pt%DIFAUXCMD
}\DIFaddend and \texttt{NetworkX}~\DIFdelbegin %DIFDELCMD < \parencite{hagberg2008}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{hagberg2008}}\hskip0pt%DIFAUXCMD
}\DIFaddend . An implementation is available at: \url{https://github.com/Neclow/GradME}.

\vspace{-1em}

==> diff/05_diff.tex <==
\subsubsection*{Tree traversal in continuous space} For any choice of label ordering, our approach admits a continuous gradient across $n!$ trees for $n$ leaves. This gradient, which can be obtained readily via automatic differentiation, can rapidly traverse tree space to find trees with a close to optimal objective value. Fig.~\ref{fig:big_jump} shows a single gradient step for the small Primates dataset~\DIFdelbegin %DIFDELCMD < \parencite{paradis2004,Yang2007-ez}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{paradis2004,Yang2007-ez}}\hskip0pt%DIFAUXCMD
}\DIFaddend . Simply subtracting the gradient from a random initial tree, followed by softmax activation, results in an almost discrete $W$ which corresponds to the best BME tree for \DIFdelbegin \DIFdel{an F81~}%DIFDELCMD < \parencite{felsenstein1981} %%%
\DIFdelend \DIFaddbegin \DIFadd{a given }\DIFaddend substitution model. \DIFaddbegin \DIFadd{Note that if more gradient steps were taken, the $W$ matrix would quickly become discrete (from Lemma~\ref{lem:discrete}). }\DIFaddend The jump taken corresponds to six subtree-prune and regraft moves~\DIFdelbegin %DIFDELCMD < \parencite{paradis2004}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{paradis2004}}\hskip0pt%DIFAUXCMD
}\DIFaddend .

For larger alignments such as the popular Eutherian dataset~\DIFdelbegin %DIFDELCMD < \parencite{Song2012-ql}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Song2012-ql}}\hskip0pt%DIFAUXCMD
}\DIFaddend , a single gradient step can result in 14 to 18 SPR moves. \DIFdelbegin \DIFdel{For comparison, picking any }\emph{\DIFdel{single}} %DIFAUXCMD
\DIFdel{subtree-prune and regraft move from the space of possible moves in a heuristic search requires $\mathcal{O}(n^2)$ moves}\DIFdelend \DIFaddbegin \DIFadd{While the number of SPR moves achieved is large, this is achieved with a substantial increase in overall computational complexity when compared to FastME}\DIFaddend . We note that the gradient step size is dependent on the data and, as expected, greatly reduces as we approach an optimum.

\input{fig/fig3}

\DIFdelbegin %DIFDELCMD < \input{tab/table2}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \input{tab/table2_1}
\DIFaddend 

\subsubsection*{A comparison to benchmark phylogenetic data sets}
Table~\ref{tab:bme_results} presents a comparison of GradME with neighbour joining (BioNJ) and FastME (subtree-prune and regraft version) over 11 popular phylogenetic benchmark datasets~\DIFdelbegin %DIFDELCMD < \parencite{Whidden2015-jn}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Whidden2015-jn}}\hskip0pt%DIFAUXCMD
}\DIFaddend . Both neighbour joining and FastME are only able to infer a minimum length unrooted tree, and therefore we compare estimates only on unrooted trees. We always initialise our algorithm with a uniform, equiprobable tree, where the starting \DIFdelbegin \DIFdel{label order is either derived from Neighbour-Joining or FastME, or from a random start }\DIFdelend \DIFaddbegin \DIFadd{taxon labelling is random }\DIFaddend and optimised using Queue Shuffle. \DIFdelbegin \DIFdel{Using Queue Shuffle therefore optimises tree topology with no sensible initial guesses}\DIFdelend \DIFaddbegin \DIFadd{We estimate tree using distances from a GTR+$\Gamma$ model estimated via maximum likelihood (see Appendix~\ref{append:est} for details)}\DIFaddend . As expected, FastME consistently outperforms BioNJ, with lower BME loss on all \DIFdelbegin \DIFdel{but one alignment. Starting from an ordering implied by BioNJ but optimising from a uniform starting tree, our algorithm matches BioNJ for three datasets but performs substantially better for the eight others. These results suggest a useful application of our algorithm is simply to improve on the greedy balanced minimum balanced evolution heuristic from a starting Neighbour-Joining tree. When starting from the ordering implied from the best tree from FastME, our algorithm achieves the same minimum, suggesting that, unlike BioNJ, FastME reliably converges to a local minimum – that is, a tree with a better objective value than those “close'' to it. Finally, implementing Queue Shuffle on a random starting order and from a uniform starting tree always achieves the best loss, and in two cases, finds a minimum smaller than FastME. For these analyses, we use an }\DIFdelend \DIFaddbegin \DIFadd{alignments. On the other hand, GradME always achieves a better or equal loss compared to FastME. We observe similar results when using different substitution models (e.g., }\DIFaddend F81\DIFdelbegin \DIFdel{substitution model with no Gamma correction to ensure simplicity, but we note performance does vary with the choice of substitution model. However, GradME does not perform worse than FastME , and always achieves a better or equal loss. Finally, we }\DIFdelend \DIFaddbegin \DIFadd{). In the two examples where GradME does better than FastME, the topological accuracy, measured by one minus the Robinson-Foulds distance~\mbox{%DIFAUXCMD
\parencite{robinson1981} }\hskip0pt%DIFAUXCMD
is close to 0.9, suggesting FastME has converged to a similar tree. We }\DIFaddend note that FastME's performance is generally worse when using the nearest neighbour interchange heuristic (instead of the SPR-based heuristic). \DIFaddbegin \DIFadd{When compared to a maximum likelihood gold standard (IQ-TREE~\mbox{%DIFAUXCMD
\parencite{minh2020}}\hskip0pt%DIFAUXCMD
), the best distance method does not recover the same tree as that from maximum likelihood, but in some cases, is very close (e.g., DS3 and DS7). Finally, we note that while GradME outperforms FastME, it is orders of magnitude slower and in most of the data sets FastME finds the same optimal tree as GradME. 
}\DIFaddend 

\subsubsection*{Rooting ultrametric trees}
Despite being applicable to the unrooted problem, our approach, at its core, works with rooted trees. As previously discussed, if we assume the existence of a distant outgroup, then the balanced minimum evolution objective can be used to optimise a rooted phylogenetic tree. In Appendix~\ref{sec:bme_rooted}, we show that, given an ultrametric unrooted tree, the optimal rooting maximises a heuristic for the root-to-tip distance in the tree. Equivalently, the optimal rooting ensures that the root is estimated to be the maximal possible distance back in time. This is not an immediately biologically plausible objective for the root. Indeed, the cornerstone of balanced minimum evolution is finding the tree of minimum length, and it hence seems counter-intuitive to require the root that is the maximum distance backwards in time (though this does in fact minimise the tree length). However, our assumption of a distant ancestor means that the root of our tree must be the point that is furthest backwards in time. In particular, this means that the evolutionary direction needs to be away from the root. By setting our root such that the root-to-tip distance is maximised, we ensure that the root satisfies this constraint. However, this property does not hold for trees that are not ultrametric - in these cases, the root will be drawn towards branches with higher mutation rates.

While this property only holds for ultrametric trees, our approach still works well for near clock-like trees. As an \DIFdelbegin \DIFdel{example}\DIFdelend \DIFaddbegin \DIFadd{experiment}\DIFaddend , we draw small (20 taxa) random ultrametric phylogenies with a total length of one, and simulate 100,000-residue protein sequences~\DIFdelbegin %DIFDELCMD < \parencite{paradis2004} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{paradis2004} }\hskip0pt%DIFAUXCMD
}\DIFaddend down these trees under an LG~\DIFdelbegin %DIFDELCMD < \parencite{Lee2015-es} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Lee2015-es} }\hskip0pt%DIFAUXCMD
}\DIFaddend model of protein evolution, assuming random uniform amino acid base frequencies. In the ultrametric cases, all taxa are equidistant to the root, which corresponds to a strict molecular clock. We add uniform noise to all branch lengths to simulate departure from a strict clock. Fig.~\ref{fig:sim_rooting} shows the Robinson-Foulds~\DIFdelbegin %DIFDELCMD < \parencite{robinson1981} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{robinson1981} }\hskip0pt%DIFAUXCMD
}\DIFaddend distance from the true tree to the \emph{midpoint-rooted} best \emph{unrooted} \DIFdelbegin \DIFdel{subtree-prune and regraft }\DIFdelend \texttt{FastME} tree \DIFaddbegin \DIFadd{(when SPR moves were used by }\texttt{\DIFadd{FastME}}\DIFadd{)}\DIFaddend , and the distance to our inferred rooted tree. We see that when the tree is ultrametric, or close to ultrametric, our approach recovers the correct rooted tree. As expected, an increase in noise leads to a decrease in topological accuracy, although our approach still performs substantially better than midpoint rooting. We note that uniform noise \DIFdelbegin \DIFdel{uniform noise }\DIFdelend is unlikely to be biologically realistic. Instead, deviations from a strict clock are more likely to be heterogeneous in certain clades or internal branches. However, for small departures, we believe our algorithm to reliably infer the correct tree and root simultaneously. 

We implement our rooting algorithm on the popular mammal data from~\DIFdelbegin %DIFDELCMD < \parencite{Song2012-ql}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Song2012-ql}}\hskip0pt%DIFAUXCMD
}\DIFaddend . We infer a rooted tree via Queue Shuffle and also midpoint root the best FastME tree. Both trees, unrooted, have the same balanced minimum evolution loss, but our rooted loss is less than the FastME midpoint rooted loss. Our rooted tree correctly identifies \textit{Gallus gallus} (red junglefowl) as the outgroup, while midpoint rooting pairs \textit{Gallus gallus} with \textit{Ornithorhynchus Anatinus} (platypus) (see Fig.~\ref{fig:Songtree} for the rooted phylogenies).

\input{fig/fig4}

\subsubsection*{Rooting the phylogeny of all jawed vertebrates}

To perform a more detailed evaluation of our framework, we tested GradME's robustness for topological inference by finding the root of the large \DIFdelbegin \DIFdel{Jawed dataset }\DIFdelend \DIFaddbegin \DIFadd{jawed vertebrates dataset from~\mbox{%DIFAUXCMD
\parencite{irisarri2017} }\hskip0pt%DIFAUXCMD
}\DIFaddend with 99 taxa and 4593 genes\DIFdelbegin \DIFdel{~}%DIFDELCMD < \parencite{irisarri2017}%%%
\DIFdelend . Given the reliance of our method on ultrametric data for inference of the root, we first made a fast measure of the ultrametricity of each gene-tree. To do this, we inferred the phylogeny of each gene using \DIFdelbegin \DIFdel{FastME}\DIFdelend \DIFaddbegin \DIFadd{GradME}\DIFaddend , followed by midpoint rooting. The coefficient of variation in root-to-tip lengths was taken as a measure of ultrametricity. We then concatenated ranked genes into supermatrices including decreasing numbers of genes, and examined the performance of \DIFdelbegin \DIFdel{FastME }\DIFdelend \DIFaddbegin \DIFadd{GradME with midpoint rooting }\DIFaddend against our method. All inferences were performed using the LG amino-acid substitution model to maintain simplicity. We placed special focus on our ability to use small portions of data for recovering the main groupings of vertebrates; these key groupings include the root separating cartilaginous (Chondrichthyes) versus boned vertebrates, ray-finned fishes (Actinopterygii), and the major groups of tetrapods and amniotes (amphibians, mammals, archosaurs, turtles, and lizards and relatives).

\DIFdelbegin \DIFdel{Strikingly, }\DIFdelend \DIFaddbegin \DIFadd{A }\DIFaddend small numbers of genes with an ultrametric signal were generally sufficient for resolving many of the major lineages of vertebrates using both \DIFdelbegin \DIFdel{FastME }\DIFdelend \DIFaddbegin \DIFadd{midpoint rooting }\DIFaddend and our approach (Fig.~\ref{fig:jawed_verts}). \DIFaddbegin \DIFadd{For larger numbers of genes, midpoint rooting and our approach are broadly similar. }\DIFaddend However, at the smallest numbers of genes (0.05\%, 2 genes), \DIFdelbegin \DIFdel{FastME }\DIFdelend \DIFaddbegin \DIFadd{midpoint rooting }\DIFaddend was unable to recover many of the early relationships among vertebrates, such as the root, monophyly of cartilaginous fishes, ray-finned fishes, Tetrapoda, or the mammals. Even small amounts of data (1460 amino-acids of 1,964,439; 0.07\% of the original data) were sufficient for GradME to resolve the root as well as every major grouping of jawed vertebrates accurately (Fig.~\ref{fig:jverts_tree}). The only exception was the controversial position of the Coelacanth, which was found to be sister of Dipnoi (lungfish) rather than the more widely accepted position as sister of Dipnoi plus Tetrapoda. While this remarkable performance under the simple LG model is in part attributed to the informative nature of highly ultrametric genes, our tree topology demonstrates the superiority of our approach in accuracy and efficiency over other fast methods in phylogenetics.


==> diff/06_diff.tex <==
We have introduced a new approach for exploring the vastness of tree space. Counterintuitively, our approach explores a much bigger space than the space of possible trees, but this larger space allows for new ways to find the best tree. The key to our method's success lies in transforming the phylogenetic tree search problem from a discrete to a continuous one, allowing us to achieve superior performance. To our knowledge, this is the first time a continuous, differentiable objective function for the inference of tree topology has been proposed, and it opens new possibilities for phylogenetic inference. Bayesian phylogenetics can be regarded as the most robust framework for inferring phylogenies, but has been to-date limited by the poor ability of random walk Metropolis-Hastings algorithms to explore tree space~\DIFdelbegin %DIFDELCMD < \parencite{Betancourt2017-fl}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Betancourt2017-fl}}\hskip0pt%DIFAUXCMD
}\DIFaddend . More efficient Hamiltonian Monte Carlo samplers have been proposed~\DIFdelbegin %DIFDELCMD < \parencite{Dinh2017-og} %%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Dinh2017-og} }\hskip0pt%DIFAUXCMD
}\DIFaddend to tackle this problem, and our framework presents a new avenue to jointly explore topology and branch lengths with efficient samplers. A remaining limitation of our approach is the need to shuffle labels to fully explore the space of all possible trees, and while the approach we use, Queue Shuffle, is mathematically and practically powerful, this step is still discrete. The possibility of permutation distributions such as the Gumbel-Sinkhorn \DIFaddbegin \DIFadd{distribution }\DIFaddend could allow for a fully differentiable algorithm. Finally, the complexity of our approach is \DIFdelbegin \DIFdel{$\mathcal{O}(n^3)$}\DIFdelend \DIFaddbegin \DIFadd{$\mathcal{O}(n^5)$}\DIFaddend , which easily allows for large phylogenies \DIFdelbegin \DIFdel{in the thousands, not for }\DIFdelend \DIFaddbegin \DIFadd{up to a thousand, but not }\DIFaddend tens of thousands. However, computation on GPUs or TPUs in parallel can facilitate computational tractability. 

A major benefit of our approach is that it naturally enables the estimation of the root node, which has been a long matter of interest in the biological sciences~\DIFdelbegin %DIFDELCMD < \parencite{Huelsenbeck2002-hb,Tria2017-cw,Naser-Khdour2022-qz}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Huelsenbeck2002-hb,Tria2017-cw,Naser-Khdour2022-qz}}\hskip0pt%DIFAUXCMD
}\DIFaddend . For genes where a strict clock is a reasonable assumption, our method of traversing tree space in large steps reliably estimates both the correct tree topology and the root. Our approach will likely be useful in settings where genetic sequences are contemporaneous and time for measurable evolution is short, such as early epidemics or nosocomial settings. However, as we showed analytically, our approach will have reduced performance when considering rate heterogeneity and departures from a strict clock. 

Tests on the relationships among jawed vertebrates demonstrate that even minimal amounts of data can be sufficient for our method to reach high accuracy in topology and root estimates. These results are consistent with previous work on large amounts of genome-scale data showing that clocklike loci to be the most suitable for phylogenetic inference~\DIFdelbegin %DIFDELCMD < \parencite{Vankan2022-xz}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Vankan2022-xz}}\hskip0pt%DIFAUXCMD
}\DIFaddend . Furthermore, our approach is effective with negligible amounts of data – where other methods are ineffective – making it a powerful addition to the existing toolkit for addressing recalcitrant questions of the tree of life.

Our approach is based on the minimum evolution principle, which has repeatedly shown to produce fast and accurate inference. Nonetheless, an interesting area for further study is to extend the continuous path length formulation to approximations of traditional phylogenetic likelihoods~\DIFdelbegin %DIFDELCMD < \parencite{felsenstein1983}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{felsenstein1983}}\hskip0pt%DIFAUXCMD
}\DIFaddend . This would be particularly beneficial for implementation in Bayesian inference, since tree topology inference is a major obstacle to large hierarchical models~\DIFdelbegin %DIFDELCMD < \parencite{Suchard2003-mh,Duchene2016-mh}%%%
\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\parencite{Suchard2003-mh,Duchene2016-mh}}\hskip0pt%DIFAUXCMD
}\DIFaddend . Our method is therefore a step towards more efficient sampling of the complex posterior distributions over tree topology. 

==> old/03_Introduction.tex <==

Phylogenetic inference, the task of reconstructing the evolutionary relationships across taxonomic units given observational data, has a wide range of theoretical and practical applications in the biological sciences, such as in biology~\parencite{cavalli1967, felsenstein2004, omeara2012} and epidemiology~\parencite{Grenfell2004-yl}, but also in linguistics~\parencite{mace2005} and cultural anthropology~\parencite{collard2006, morrison2014}. In particular, the COVID-19 pandemic has catalysed research efforts to develop efficient tools and methods in phylogenetics~\parencite{lemoine2021, otoole2021, attwood2022, sanderson2022, turakhia2022, voznica2022, demaio2023}. For biological problems, tree inference is primarily informed by molecular sequence data (i.e., nucleotide or amino acid sequences), for which an extensive body of literature exists~\parencite{sanderson2002, yang2006, yang2012}. Other sources of biological data such as morphology~\parencite{Lee2015-es}, fossils~\parencite{Morlon2011-pe}, and auditory communication in animals~\parencite{arato2021} can also be used as input. Yet despite an explosion in data available for millions of taxonomic units, as seen during the recent pandemic, we are still unable to effectively explore the gigantic parameter spaces involved during inference.

Two key parameters considered when inferring a phylogenetic tree include the \emph{topology}, the branching pattern that specifies the evolutionary relationships between operational taxonomic units, and \emph{branch lengths}, the amount of evolutionary divergence that occurred between the branching events. A substantial amount of research has been conducted on how to parameterise branch lengths~\parencite{bromham2003, dosreis2016}, especially through the use of molecular clocks~\parencite{zuckerkandl1962}. Conversely, relatively little progress has been made on methods for exploring the massive spaces of possible tree topologies. This is a fundamental challenge for inference given its combinatorial complexity: for $n$ taxa, there are $(2n-3)!!$ possible rooted tree arrangements. This means that even a small dataset of 10 taxa can be enumerated by 34 million unique rooted trees. Moreover, finding the optimal tree is NP-hard for all major optimality criteria (e.g., maximum parsimony~\parencite{foulds1982}, minimum evolution~\parencite{day1986}, maximum likelihood~\parencite{roch2006}). Methods such as linear programming~\parencite{catanzaro2012} or branch and bound~\parencite{Hendy1982-dy} can provide exact solutions, but are practically limited to problems with $\approx$ 15 or fewer taxa. To overcome these challenges, the overwhelming majority of state-of-the-art software (e.g., \texttt{MrBayes}~\parencite{huelsenbeck2001}, \texttt{PAUP}~\parencite{Wilgenbusch2003-mu}, \texttt{BEAST}~\parencite{Drummond2007-za}, \texttt{PAML}~\parencite{Yang2007-ez}, \texttt{RAxML}(\texttt{-NG})~\parencite{stamatakis2014, kozlov2019}, \texttt{FastME}~\parencite{lefort2015}, \texttt{IQ-TREE}~\parencite{nguyen2015, minh2020}) rely on hand-engineered search heuristics to perform tree topology optimisation.

\input{fig/fig1}

The most popular of these methods still have several limitations, and this includes heuristics based on subtree pruning and regrafting (SPR) and tree bisection and reconnection (TBR) operations, which have empirically been shown to be the best available methods for exploring tree topology space~\parencite{stamatakis2014, Park2010-zq}. First, the computational cost of such heuristic approaches scales poorly as the number of taxa increases. For instance, exhaustive exploration of single SPR operations is quadratic in complexity, and paired changes is quartic. The computational cost of SPR is further compounded by large memory requirements for tracking the changes from one iteration to the next. Second, all the aforementioned tree arrangements are prone to convergence to poor local minima~\parencite{sanderson2011} due to the inability of heuristic operations to provide sufficient directions of change to a better tree. This phenomenon is exacerbated when concatenating multiple genes in a supermatrix approach~\parencite{rokas2003, dequeiroz2007}, and when using genomic-scale data sets that lead to further computational demands.



We address these shortcomings by proposing a new paradigm for tree topology inference, expanding the problem space using a continuous rather than discrete parameterisation of a phylogenetic tree. To our knowledge, aside from considering metrics (e.g., distances in tree space)~\parencite{St_John2017-vq,Dinh2017-og,Billera2001-il}, performing topological search in a continuous tree space has not been attempted. Furthermore, very few approaches have made use of gradient-based tree proposals~\parencite{zhang2018, nesterenko2022,Dinh2017-og}.  Although maximum likelihood and Bayesian inference criteria are more popular and generally considered state-of-the-art~\parencite{huelsenbeck2001, stamatakis2014, Drummond2007-za, minh2020, Wilgenbusch2003-mu, ayres2012}, our framework optimises tree topology under a balanced minimum evolution (BME) criterion~\parencite{Pauplin2000-vk,Desper2002-uy} using dissimilarity matrices as an input. This criterion is well-principled~\parencite{Kidd1971-sk} theoretically can match the performance of maximum likelihood approaches~\parencite{Roch2010-uj}. This framing of the minimum evolution criterion~\parencite{Kidd1971-sk, Rzhetsky1992-qj} has also been proven to be statistically consistent~\parencite{Desper2004-ij,felsenstein2004} and has repeatedly shown outstanding performance in a range of settings~\parencite{Kuhner1994-cf, kumar2000, Gascuel2006-sr, lefort2015}. 

To better explore the space of possible trees, we expand the space over which we need to search. Consequently, we use a continuous representation of a phylogenetic tree~\parencite{penn2023} to greatly improve the ability to search parts of this space. Appealing to a common analogy that casts the optimal tree search problem as finding a needle in a haystack, our approach observes a much bigger haystack, but the hay is in very large bundles, many of whom have a needle, and for these bundles we have access to a (weak) magnet. Providing details to this analogy, the size of the usual phylogenetic haystack with $n$ taxa is $(2n-3)!!$~\parencite{Felsenstein1978-qc}, while we search a much larger haystack of size $(n!)^2$. There are $n!$ bundles in this larger haystack, each of which contains $n!$ trees, but for any tree, $2^{n-1}$ bundles will contain that tree. Although the proportion of bundles containing a needle shrinks exponentially, we propose a novel approach (Queue Shuffle) that chooses bundles that should be closer to one with a needle. For any given bundle, we also introduce a continuous objective function that can be efficiently traversed using gradient descent approaches (the weak magnet) developed for large-scale machine learning problems~\parencite{Kingma2014-ow, loshchilov2018, shazeer2018}. This continuous objective facilitates enormous changes to tree topology in a single step in a direction that improves the objective function. After searching any given bundle using the continuous objective, we use Queue Shuffle, which improves the switch towards the next bundle to search. Our counterintuitive approach, called GradME, offers a powerful alternative to the existing heuristic methods used for topological inference, outperforming the current state-of-the-art with an overall complexity comparable to neighbour joining ($\mathcal{O}(n^3)$).


==> old/04_Methods.tex <==
\subsubsection*{An ordered bijection to tree space}~Previously, we introduced Phylo2Vec~\parencite{penn2023}, a novel bijection between the space of trees and a space of integer vectors. In contrast to other bijections such as Prüfer codes~\parencite{C_Chen2000-ak} or permutation matchings~\parencite{diaconis1998}, changes in Phylo2Vec correspond to smooth changes in the tree space, e.g., single changes in a Phylo2Vec vector correspond to a limited set of SPR changes. 

Here, we focus on the notion of \emph{ordered trees} from~\parencite{penn2023}, where it is possible to construct a tree from its vector in linear ($\mathcal{O}(n)$) time. An ordered tree can be thought of as a birth process, where when a birth occurs, the original node continues to live and retains its label, while the new node receives an incremented label. Accordingly, we introduce an equivalent but more intuitive tree construction process for these ordered trees. We begin with two leaf nodes and two edges labelled 0 and 1. We then append nodes by joining them, \emph{in order}, to edges connecting leaf nodes to the tree. In Fig.~\ref{fig:ltr}, we first append node 2 to its label edge 0, creating a new internal node and a pair of new edges. The new edge joining node 2 to the tree is labelled as edge 2. We then append node 3 to edge 2, again creating a new internal node and two new edges. This tree construction process can be summarised by a single vector $\boldsymbol{v}$, with $v_0 = v_1 = 0$ and, for $m \geq 2$, $v_m$ being the label of the edge to which node $m$ is appended. Each index in $v_m$ is subject to the simple constraint:

\begin{align}
\label{eq:disc}
    & v_0 = v_1 = 0 \quad \text{and} \\ 
    & v_m \in \{0,1,...,m-1\} \quad \forall \quad m \geq 2 \nonumber
\end{align}
which is equivalent to the definition of ordered trees in~\parencite{penn2023}. It is proved in Appendix~\ref{sec:ordered} that for ordered $\boldsymbol{v}$, the algorithm presented above and the more general algorithm in~\parencite{penn2023} produce equivalent trees. 

\input{fig/fig2}

\subsubsection*{A continuous representation of a tree}
We introduce a square matrix $W$ which gives the distribution of a random ordered vector $\boldsymbol{V}$ with independent entries such that $W_{ij} = \mathbb{P}(V_i = j)$. Given Eq.~\ref{eq:disc}, $W$ is a lower-triangular, stochastic matrix (row sums to 1). $W$ is designed to be a continuous representation of a phylogenetic tree, and can probabilistically represent any \emph{ordered} phylogenetic tree (a space of $n!$ trees). A simple approach to determining the best single tree from $W$ is to take the column-wise argmax, yielding a single tree $\boldsymbol{v}$.

\subsubsection*{Queue Shuffle: changing orderings to explore all the tree space}
The number of ordered trees, $n!$, is substantially smaller than the possible number of trees, $(2n-3)!!$ (although with a comparable growth pattern in $n$), and hence, the optimal ordered tree is likely to be close to, but not exactly equal to, the true optimal tree. 

To fully explore tree space, we randomly change the labels of the leaf nodes in the optimal ordered tree using a novel approach we call the \textit{Queue Shuffle} (full details in Appendix~\ref{sec:queue_shuffle}). Shuffling amounts to choosing a permutation $\sigma$ on $\{0,1...,n-1\}$ such that the leaf with name $N_i$ now has label $\sigma(i)$. We call this an \textit{ordering} of the leaf nodes.

Each different ordering changes the explorable space of ordered trees. Thus, once an ordering is chosen, one can re-optimise an objective function $F(W)$ in this new space of ordered trees (note that the previous optimal tree is still in this space and so, provided it finds the true optimal ordered tree, it will have an objective value no worse than the previous tree). This process is then repeated, re-ordering the tree and re-optimising in the new space, until the best found tree does not change for a certain number of iterations. In practice, only ten to twenty iterations are needed from some random starting order, and less if a sensible start (such as from a neighbour joining tree) is used.

A given tree is in the space of ordered trees for at least $2^{n-1}$ orderings. This means that we do not need to find a single optimal ordering, but have exponentially many which will return the true optimal tree. Very loosely considered, being able to explore $n!$ tree space reliably and efficiently with continuous optimisation, Queue Shuffle reduces the inferential task to one that is exponential.

\subsubsection*{Why does Queue Shuffle work?}

While the number of optimal orderings grows exponentially, their proportion tends quickly to zero as $n$ grows. It is therefore, perhaps, surprising that we are able to find an optimal ordering so quickly from merely tens of shuffles. The proportion of optimal orderings (approximately the ratio of ordered trees to total trees, $\frac{(n-1)!}{(2n-3)!!}$) ranges from $8\times 10^{-4}$ in our smallest dataset (14 taxa) to $6\times 10^{-29}$ in the largest (99 taxa).

However, our algorithm is able to find these optimal orderings because the Queue Shuffle does not choose the new ordering uniformly over the space of orderings (which is $n!$ large). Instead, the distribution depends on the structure of the tree and therefore facilitates sensible proposals. For example, nodes which are close to the root are always given low labels, meaning that they will also be close to the root in a high proportion of the trees in the new space of ordered trees (cf. Appendix~\ref{sec:queue_shuffle}).

When a good tree is found in some ordered space, it is reasonable to expect a better tree will retain similarities with the good tree, and the Queue Shuffle allows for these trees to be explored. Theorem 1 in Appendix~\ref{sec:queue_shuffle} formalises the \textit{swapping property} of the Queue Shuffle, illustrated in Fig.~\ref{fig:swap}. Given any pair of subtrees which are connected to the tree by two nodes that share an edge, the swapping property states that, with at least probability $\frac{1}{4}$, a tree that is identical to the previous optimum, with the exception that these two subtrees are swapped, will be in the new space of ordered trees. This ensures that this new space  contains many sensible proposal trees. Moreover, the fact that this probability is bounded below by a fixed constant, independent of the size of the phylogeny, is a surprising, and powerful property: it means that there is a sense of continuity when moving between ordered tree spaces. 

\subsubsection*{Balanced minimum evolution}~Popular objective functions for inferring the best tree given some data include maximum parsimony~\parencite{Fitch1967-dr}, maximum likelihood~\parencite{felsenstein1983} and minimum evolution~\parencite{Saitou1987-wg}. Of these three, only maximum likelihood and minimum evolution are provably statistically consistent~\parencite{Desper2004-ij,felsenstein2004} (maximum parsimony can be inconsistent under certain conditions~\parencite{Felsenstein1978-jt}). For small to moderate sized phylogenies, maximum likelihood (and Bayesian extensions) is generally considered state-of-the-art~\parencite{stamatakis2014, Drummond2007-za, minh2020, Wilgenbusch2003-mu}, but approaches based on minimum evolution have also consistently shown to yield comparable performance~\parencite{Kuhner1994-cf, Gascuel2006-sr, lefort2015, kumar2000, roch2006}. The first introductions of the minimum evolution paradigm~\parencite{Kidd1971-sk, Rzhetsky1992-qj} sought to express evolutionary relationships through dissimilarity. They proved that, given unbiased estimates of the true evolutionary distances, the true phylogeny has an expected length shorter than any other possible phylogeny – thereby establishing a principled objective criterion. Currently, the best performing minimum evolution approach is that of balanced minimum evolution (BME)~\parencite{Pauplin2000-vk,Desper2002-uy} (with the widely used software implementation \texttt{FastME}~ \parencite{lefort2015}). Given $D_{ij}$, the distance between two taxa $i$,$j$, (where this distance could be based on morphology, molecular sequences etc.) and $e_{ij}$, the number of branches in the path between taxa $i$ and $j$ (the path length~\parencite{Semple2004-my}), the objective function for a given tree $T$ is:
\begin{equation}
    \mathcal{L}(T) = \sum_{i,j}D_{ij}2^{-e_{ij}}
    \label{eq:bme_objective}
\end{equation}
This objective can be computed in a numerically stable fashion using the log-sum-exp trick. A widely used approach to estimate the optimal tree greedily~\parencite{Desper2004-ij, Gascuel2006-sr} is the neighbour joining method~\parencite{Saitou1987-wg}. When neighbour joining is based on an additive distance measure, it reconstructs a unique tree, but still performs well with near-additive trees~\parencite{Atteson1999-jd} and under small perturbations in the data~\parencite{Mihaescu2009-es}. However, despite these highly favourable properties, further heuristic optimisation on a neighbour joining tree utilising subtree-prune and regrafting have proven to be even more accurate~\parencite{lefort2015}. Once a tree topology is found, quadratic algorithms exist for estimating the branch lengths~\parencite{Mihaescu2008-bo} as well as efficient approaches for molecular clock dating~\parencite{To2016-vd}.

\subsubsection*{Balanced minimum evolution for rooted trees}

Inference using BME is almost always restricted to unrooted trees~\parencite{Semple2004-my} with rooting chosen after inference through heuristics (e.g., midpoint rooting) or via a molecular clock (e.g., for serially sampled data). However, it is often of interest to find the optimal rooted tree for a set of taxa, as this provides extra biological context.

In an unrooted tree, the BME objective function (Eq.~\ref{eq:bme_objective}) provides an efficient way of calculating the total length of a tree where the branch lengths are the least squares estimators for approximating each $D_{ij}$ with the distance from nodes $i$ to $j$ in the tree. However, this result does not hold in a rooted tree, as the addition of a root changes some path lengths.

To remedy this, we consider adding a hypothetical and very distant, root (as node $n$) into the tree and finding the optimal unrooted tree with these $n+1$ taxa. We can create a rooted tree by removing node $n$ and, as we know that node $n$ evolved first, this will be the root of the original $n$ taxa. Moreover, we show in Appendix~\ref{sec:bme_rooted} that, to leading order, the BME objective applied to this rooted tree differs only by a constant from the BME objective applied to the unrooted tree with $n+1$ taxa. Thus, BME provides a sensible method for finding the optimal rooted tree and can be sensibly applied directly to a rooted topology. However, as discussed in detail in Appendix~\ref{sec:bme_rooted}, it will struggle to find the correct root of trees that are not ultrametric as the root will be drawn towards taxa that are more distant from the root.

\subsubsection*{Gradient-based optimisation using the BME criterion}
Defining $f(\boldsymbol{v})$ to be the BME objective function for the tree generated by $\boldsymbol{v}$, we then create a continuous objective, $F(W)$ by $    F(W) = \mathbb{E}\bigg[f(\boldsymbol{V})\bigg]$. We present in Appendix~\ref{sec:continuous_edge} a novel method for calculating this objective function in cubic time ($\mathcal{O}(n^3)$; where $n$ is the number of taxa). We can perform inference on this objective for both rooted and unrooted trees.

An important property of our continuous objective function is that there is always a minimum at a “discrete tree'' – that is, at a matrix $W$ where for each row, one value is 1 and all the others are 0 (e.g., see Fig.~\ref{fig:big_jump}). Moreover, the objective function is a polynomial function of the entries of $W$ and is linear in each fixed entry (that is, the diagonal entries of $\nabla^2 F$ are zero), making it easy to differentiate analytically, numerically or automatically. Using state-of-the-art automatic differentiation~\parencite{jax2018github}, gradient descent can be used to efficiently minimize $F$ and find the optimal \textit{ordered} tree. 

We refer the resulting system, combining the continuous tree representation, Queue Shuffle reordering, and the gradient-based optimisation framework using BME, as \textsb{GradME}.

\input{tab/table1}

\subsubsection*{Evaluation} We evaluate GradME on a diverse corpus of 14 empirical molecular sequence datasets (Table~\ref{tab:data}). The first 11 are commonly used to assess phylogenetic inference performance~\parencite{Whidden2015-jn}, whereas the last three were used to assess inference on rooted trees. For each dataset, we start from a random tree and optimise the $W$ matrix to a tolerance of 1e-10 using gradient descent with Adafactor~\parencite{shazeer2018} optimisation. The distance matrix $D$ is computed using the F81 substitution model for DNA~\parencite{felsenstein1981}, and LG~\parencite{Le2008-ut} for amino acids. Jukes-Cantor~\parencite{jukes1969} and TN93~\parencite{tamura1993} models were also considered for DNA, while stochastic gradient descent (SGD), RMSprop~\parencite{tieleman2012}, and AdamW~\parencite{Kingma2014-ow, loshchilov2018} were also considered for optimisation (see Fig.~\ref{fig:convergence_analysis}). As a baseline, we compute the mean BME loss over 50 random uniform trees, sampled using Phylo2Vec~\parencite{penn2023}. To fairly assess the performance of GradME, we compare our framework to two well-established distance-based methods: \texttt{BioNJ}~\parencite{gascuel1997}, based on the neighbour joining algorithm~\parencite{saitou1987}, and \texttt{FastME}~\parencite{lefort2015}, based on balanced minimum evolution.

\vspace{-1em}

\subsubsection*{Implementation} Implementation of the BME criterion and of the optimisation framework was written in Python using \texttt{Jax}~\parencite{jax2018github} and \texttt{Optax}~\parencite{deepmind2020}. Optimisation was performed on a Xeon 2.30GHz (CPU; Intel Corporation) or on a single GeForce GTX 1080 (GPU; Nvidia Corporation). Evaluation of the \texttt{BioNJ}~\parencite{gascuel1997} and \texttt{FastME}~\parencite{lefort2015} methods was performed via the R package \texttt{ape}~\parencite{paradis2004} using \texttt{rpy2}~\parencite{rpy2}. Tree manipulation and visualisation scripts were written using \texttt{ete3}~\parencite{huerta2016} and \texttt{NetworkX}~\parencite{hagberg2008}. An implementation is available at: \url{https://github.com/Neclow/GradME}.

\vspace{-1em}


==> old/05_Results.tex <==
\subsubsection*{Tree traversal in continuous space} For any choice of label ordering, our approach admits a continuous gradient across $n!$ trees for $n$ leaves. This gradient, which can be obtained readily via automatic differentiation, can rapidly traverse tree space to find trees with a close to optimal objective value. Fig.~\ref{fig:big_jump} shows a single gradient step for the small Primates dataset~\parencite{paradis2004,Yang2007-ez}. Simply subtracting the gradient from a random initial tree, followed by softmax activation, results in an almost discrete $W$ which corresponds to the best BME tree for an F81~\parencite{felsenstein1981} substitution model. The jump taken corresponds to six subtree-prune and regraft moves~\parencite{paradis2004}.

For larger alignments such as the popular Eutherian dataset~\parencite{Song2012-ql}, a single gradient step can result in 14 to 18 SPR moves. For comparison, picking any \emph{single} subtree-prune and regraft move from the space of possible moves in a heuristic search requires $\mathcal{O}(n^2)$ moves. We note that the gradient step size is dependent on the data and, as expected, greatly reduces as we approach an optimum.

\input{fig/fig3}

\input{tab/table2}

\subsubsection*{A comparison to benchmark phylogenetic data sets}
Table~\ref{tab:bme_results} presents a comparison of GradME with neighbour joining (BioNJ) and FastME (subtree-prune and regraft version) over 11 popular phylogenetic benchmark datasets~\parencite{Whidden2015-jn}. Both neighbour joining and FastME are only able to infer a minimum length unrooted tree, and therefore we compare estimates only on unrooted trees. We always initialise our algorithm with a uniform, equiprobable tree, where the starting label order is either derived from Neighbour-Joining or FastME, or from a random start and optimised using Queue Shuffle. Using Queue Shuffle therefore optimises tree topology with no sensible initial guesses. As expected, FastME consistently outperforms BioNJ, with lower BME loss on all but one alignment. Starting from an ordering implied by BioNJ but optimising from a uniform starting tree, our algorithm matches BioNJ for three datasets but performs substantially better for the eight others. These results suggest a useful application of our algorithm is simply to improve on the greedy balanced minimum balanced evolution heuristic from a starting Neighbour-Joining tree. When starting from the ordering implied from the best tree from FastME, our algorithm achieves the same minimum, suggesting that, unlike BioNJ, FastME reliably converges to a local minimum – that is, a tree with a better objective value than those “close'' to it. Finally, implementing Queue Shuffle on a random starting order and from a uniform starting tree always achieves the best loss, and in two cases, finds a minimum smaller than FastME. For these analyses, we use an F81 substitution model with no Gamma correction to ensure simplicity, but we note performance does vary with the choice of substitution model. However, GradME does not perform worse than FastME, and always achieves a better or equal loss. Finally, we note that FastME's performance is generally worse when using the nearest neighbour interchange heuristic (instead of the SPR-based heuristic).

\subsubsection*{Rooting ultrametric trees}
Despite being applicable to the unrooted problem, our approach, at its core, works with rooted trees. As previously discussed, if we assume the existence of a distant outgroup, then the balanced minimum evolution objective can be used to optimise a rooted phylogenetic tree. In Appendix~\ref{sec:bme_rooted}, we show that, given an ultrametric unrooted tree, the optimal rooting maximises a heuristic for the root-to-tip distance in the tree. Equivalently, the optimal rooting ensures that the root is estimated to be the maximal possible distance back in time. This is not an immediately biologically plausible objective for the root. Indeed, the cornerstone of balanced minimum evolution is finding the tree of minimum length, and it hence seems counter-intuitive to require the root that is the maximum distance backwards in time (though this does in fact minimise the tree length). However, our assumption of a distant ancestor means that the root of our tree must be the point that is furthest backwards in time. In particular, this means that the evolutionary direction needs to be away from the root. By setting our root such that the root-to-tip distance is maximised, we ensure that the root satisfies this constraint. However, this property does not hold for trees that are not ultrametric - in these cases, the root will be drawn towards branches with higher mutation rates.

While this property only holds for ultrametric trees, our approach still works well for near clock-like trees. As an example, we draw small (20 taxa) random ultrametric phylogenies with a total length of one, and simulate 100,000-residue protein sequences~\parencite{paradis2004} down these trees under an LG~\parencite{Lee2015-es} model of protein evolution, assuming random uniform amino acid base frequencies. In the ultrametric cases, all taxa are equidistant to the root, which corresponds to a strict molecular clock. We add uniform noise to all branch lengths to simulate departure from a strict clock. Fig.~\ref{fig:sim_rooting} shows the Robinson-Foulds~\parencite{robinson1981} distance from the true tree to the \emph{midpoint-rooted} best \emph{unrooted} subtree-prune and regraft \texttt{FastME} tree, and the distance to our inferred rooted tree. We see that when the tree is ultrametric, or close to ultrametric, our approach recovers the correct rooted tree. As expected, an increase in noise leads to a decrease in topological accuracy, although our approach still performs substantially better than midpoint rooting. We note that uniform noise  uniform noise is unlikely to be biologically realistic. Instead, deviations from a strict clock are more likely to be heterogeneous in certain clades or internal branches. However, for small departures, we believe our algorithm to reliably infer the correct tree and root simultaneously. 

We implement our rooting algorithm on the popular mammal data from~\parencite{Song2012-ql}. We infer a rooted tree via Queue Shuffle and also midpoint root the best FastME tree. Both trees, unrooted, have the same balanced minimum evolution loss, but our rooted loss is less than the FastME midpoint rooted loss. Our rooted tree correctly identifies \textit{Gallus gallus} (red junglefowl) as the outgroup, while midpoint rooting pairs \textit{Gallus gallus} with \textit{Ornithorhynchus Anatinus} (platypus) (see Fig.~\ref{fig:Songtree} for the rooted phylogenies).

\input{fig/fig4}

\subsubsection*{Rooting the phylogeny of all jawed vertebrates}

To perform a more detailed evaluation of our framework, we tested GradME's robustness for topological inference by finding the root of the large Jawed dataset with 99 taxa and 4593 genes~\parencite{irisarri2017}. Given the reliance of our method on ultrametric data for inference of the root, we first made a fast measure of the ultrametricity of each gene-tree. To do this, we inferred the phylogeny of each gene using FastME, followed by midpoint rooting. The coefficient of variation in root-to-tip lengths was taken as a measure of ultrametricity. We then concatenated ranked genes into supermatrices including decreasing numbers of genes, and examined the performance of FastME against our method. All inferences were performed using the LG amino-acid substitution model to maintain simplicity. We placed special focus on our ability to use small portions of data for recovering the main groupings of vertebrates; these key groupings include the root separating cartilaginous (Chondrichthyes) versus boned vertebrates, ray-finned fishes (Actinopterygii), and the major groups of tetrapods and amniotes (amphibians, mammals, archosaurs, turtles, and lizards and relatives).

Strikingly, small numbers of genes with an ultrametric signal were generally sufficient for resolving many of the major lineages of vertebrates using both FastME and our approach (Fig.~\ref{fig:jawed_verts}). However, at the smallest numbers of genes (0.05\%, 2 genes), FastME was unable to recover many of the early relationships among vertebrates, such as the root, monophyly of cartilaginous fishes, ray-finned fishes, Tetrapoda, or the mammals. Even small amounts of data (1460 amino-acids of 1,964,439; 0.07\% of the original data) were sufficient for GradME to resolve the root as well as every major grouping of jawed vertebrates accurately (Fig.~\ref{fig:jverts_tree}). The only exception was the controversial position of the Coelacanth, which was found to be sister of Dipnoi (lungfish) rather than the more widely accepted position as sister of Dipnoi plus Tetrapoda. While this remarkable performance under the simple LG model is in part attributed to the informative nature of highly ultrametric genes, our tree topology demonstrates the superiority of our approach in accuracy and efficiency over other fast methods in phylogenetics.


==> old/06_Discussion.tex <==
We have introduced a new approach for exploring the vastness of tree space. Counterintuitively, our approach explores a much bigger space than the space of possible trees, but this larger space allows for new ways to find the best tree. The key to our method's success lies in transforming the phylogenetic tree search problem from a discrete to a continuous one, allowing us to achieve superior performance. To our knowledge, this is the first time a continuous, differentiable objective function for the inference of tree topology has been proposed, and it opens new possibilities for phylogenetic inference. Bayesian phylogenetics can be regarded as the most robust framework for inferring phylogenies, but has been to-date limited by the poor ability of random walk Metropolis-Hastings algorithms to explore tree space~\parencite{Betancourt2017-fl}. More efficient Hamiltonian Monte Carlo samplers have been proposed~\parencite{Dinh2017-og} to tackle this problem, and our framework presents a new avenue to jointly explore topology and branch lengths with efficient samplers. A remaining limitation of our approach is the need to shuffle labels to fully explore the space of all possible trees, and while the approach we use, Queue Shuffle, is mathematically and practically powerful, this step is still discrete. The possibility of permutation distributions such as the Gumbel-Sinkhorn could allow for a fully differentiable algorithm. Finally, the complexity of our approach is $\mathcal{O}(n^3)$, which easily allows for large phylogenies in the thousands, not for tens of thousands. However, computation on GPUs or TPUs in parallel can facilitate computational tractability. 

A major benefit of our approach is that it naturally enables the estimation of the root node, which has been a long matter of interest in the biological sciences~\parencite{Huelsenbeck2002-hb,Tria2017-cw,Naser-Khdour2022-qz}. For genes where a strict clock is a reasonable assumption, our method of traversing tree space in large steps reliably estimates both the correct tree topology and the root. Our approach will likely be useful in settings where genetic sequences are contemporaneous and time for measurable evolution is short, such as early epidemics or nosocomial settings. However, as we showed analytically, our approach will have reduced performance when considering rate heterogeneity and departures from a strict clock. 

Tests on the relationships among jawed vertebrates demonstrate that even minimal amounts of data can be sufficient for our method to reach high accuracy in topology and root estimates. These results are consistent with previous work on large amounts of genome-scale data showing that clocklike loci to be the most suitable for phylogenetic inference~\parencite{Vankan2022-xz}. Furthermore, our approach is effective with negligible amounts of data – where other methods are ineffective – making it a powerful addition to the existing toolkit for addressing recalcitrant questions of the tree of life.

Our approach is based on the minimum evolution principle, which has repeatedly shown to produce fast and accurate inference. Nonetheless, an interesting area for further study is to extend the continuous path length formulation to approximations of traditional phylogenetic likelihoods~\parencite{felsenstein1983}. This would be particularly beneficial for implementation in Bayesian inference, since tree topology inference is a major obstacle to large hierarchical models~\parencite{Suchard2003-mh,Duchene2016-mh}. Our method is therefore a step towards more efficient sampling of the complex posterior distributions over tree topology. 

==> old/table2.tex <==
\begin{table*}[htbp]
\centering
\caption{Log balanced minimum evolution loss scores for 11 phylogenetic benchmark datasets. Lower is better. Scores from BioNJ and FastME were obtained following the implementations in \texttt{ape}~\cite{paradis2004}. Our approach always starts from a random uniform tree, but requires a taxon labelling ordering. We show the performance of our approach starting from a BioNJ ordering, FastME ordering, and a random ordering, optimised by Queue Shuffle. The baseline was obtained by uniformly sampling 50 random trees and obtaining their BME loss (shown: mean $\pm$ SD). The best performing approaches for each dataset are denoted in bold.}
\begin{tabular}{l@{\hspace{10pt}}*5{r}@{\hspace{10pt}}c}
\toprule
Dataset & \multicolumn{1}{c}{Baseline} & \multicolumn{2}{c}{No ordering} & \multicolumn{2}{c}{With ordering} \\
        & \multicolumn{1}{c}{Random tree} & \multicolumn{1}{c}{BioNJ} & \multicolumn{1}{c}{FastME} & \multicolumn{1}{c}{BioNJ} & \multicolumn{1}{c}{FastME} & \multicolumn{1}{c}{GradME (ours)} \\
\midrule
DS1  & -0.609 $\pm$ 0.043 & -1.18334 & \textsb{-1.19145} & -1.18334         & \textsb{-1.19145} & \textsb{-1.19145} \\ 
DS2  & 1.279 $\pm$ 0.021 & 0.97379  & 0.97408           & 0.97379          & 0.97408           & \textsb{ 0.97349}  \\ 
DS3  & 1.586 $\pm$ 0.023 & 1.23596  & \textsb{1.23567}  & 1.23589          & \textsb{1.23567}  & \textsb{ 1.23567}  \\ 
DS4  & 1.132 $\pm$ 0.020 & 0.67644  & \textsb{0.67430}  & 0.67565          & \textsb{0.67430}  & \textsb{ 0.67430}  \\ 
DS5  & 1.708 $\pm$ 0.014 & 1.32536  & \textsb{1.32003}  & 1.32381          & \textsb{1.32003}  & \textsb{ 1.32003}  \\ 
DS6  & 0.366 $\pm$ 0.024 & -0.48565 & -0.48739          & -0.48715         & -0.48739          & \textsb{-0.48886} \\ 
DS7  & 1.947 $\pm$ 0.020 & 1.29616  & \textsb{1.29433}  & 1.29616          & \textsb{1.29433}  & \textsb{ 1.29433}  \\ 
DS8  &  1.029 $\pm$ 0.017 & 0.26538  & \textsb{0.25609}  & 0.26294          & \textsb{0.25609}  & \textsb{ 0.25609}  \\ 
DS9  & -0.161 $\pm$ 0.022 & -0.97842 & \textsb{-0.97989} & -0.97860         & \textsb{-0.97989} & \textsb{-0.97989} \\ 
DS10 & 0.892 $\pm$ 0.017 & 0.09618  & \textsb{0.09334}  & 0.09483          & \textsb{0.09334}  & \textsb{ 0.09334}  \\ 
DS11 & 1.152 $\pm$ 0.032 & -0.07904 & \textsb{-0.08090} & -0.07985         & \textsb{-0.08090} & \textsb{-0.08090} \\ 
\bottomrule
\end{tabular}
\label{tab:bme_results}
\end{table*}

% \begin{table*}[htbp]
% \centering
% \caption{Log balanced minimum evolution loss scores for 11 phylogenetic benchmark datasets. Lower is better. Scores from BioNJ and FastME were obtained following the implementations in \texttt{ape}~\cite{paradis2004}. Our approach always starts from a random uniform tree, but requires a taxon labelling ordering. We show the performance of our approach starting from a BioNJ ordering, FastME ordering, and a random ordering, optimised by Queue Shuffle. The baseline was obtained by uniformly sampling 50 random trees and obtaining their BME loss (shown: mean $\pm$ SD). The best performing approaches for each dataset are denoted in bold.}
% \begin{tabular}{l@{\hspace{10pt}}*5{r}@{\hspace{10pt}}c}
% \toprule
% Dataset & \multicolumn{1}{c}{Baseline} & \multicolumn{2}{c}{No ordering} & \multicolumn{2}{c}{With ordering} \\
%         & \multicolumn{1}{c}{Random tree} & \multicolumn{1}{c}{BioNJ} & \multicolumn{1}{c}{FastME} & \multicolumn{1}{c}{BioNJ} & \multicolumn{1}{c}{FastME} & \multicolumn{1}{c}{Queue Shuffle (ours)} \\
% \midrule
% DS1  & -0.583 $\pm$ 0.043 & -1.18334 & \textsb{-1.19145} & -1.18334         & \textsb{-1.19145} & \textsb{-1.19145} \\ 
% DS2  & 1.311 $\pm$ 0.023 & 0.97379  & 0.97408           & 0.97379          & 0.97408           & \textsb{ 0.97349}  \\ 
% DS3  & 1.614 $\pm$ 0.020 & 1.23596  & \textsb{1.23567}  & 1.23589          & \textsb{1.23567}  & \textsb{ 1.23567}  \\ 
% DS4  & 1.160 $\pm$ 0.022 & 0.67644  & \textsb{0.67430}  & 0.67565          & \textsb{0.67430}  & \textsb{ 0.67430}  \\ 
% DS5  & 1.728 $\pm$ 0.016 & 1.32536  & \textsb{1.32003}  & 1.32381          & \textsb{1.32003}  & \textsb{ 1.32003}  \\ 
% DS6  & 0.383 $\pm$ 0.031 & -0.48565 & -0.48739          & -0.48715         & -0.48739          & \textsb{-0.48886} \\ 
% DS7  & 1.971 $\pm$ 0.024 & 1.29616  & \textsb{1.29433}  & 1.29616          & \textsb{1.29433}  & \textsb{ 1.29433}  \\ 
% DS8  &  1.051 $\pm$ 0.016 & 0.26538  & \textsb{0.25609}  & 0.26294          & \textsb{0.25609}  & \textsb{ 0.25609}  \\ 
% DS9  & -0.144 $\pm$ 0.019 & -0.97842 & \textsb{-0.97989} & -0.97860         & \textsb{-0.97989} & \textsb{-0.97989} \\ 
% DS10 & -0.906 $\pm$ 0.021 & 0.09618  & \textsb{0.09334}  & 0.09483          & \textsb{0.09334}  & \textsb{ 0.09334}  \\ 
% DS11 & 1.172 $\pm$ 0.032 & -0.07904 & \textsb{-0.08090} & -0.07985         & \textsb{-0.08090} & \textsb{-0.08090} \\ 
% \bottomrule
% \end{tabular}
% \label{tab:bme_results}
% \end{table*}
